Feature Enhancer Segmentation Network (FES-Net) for Vessel Segmentation

Diseases such as diabetic retinopathy and age-related macular degeneration pose a significant risk to vision, highlighting the importance of precise segmentation of retinal vessels for the tracking and diagnosis of progression. However, existing vessel segmentation methods that heavily rely on encoder-decoder structures struggle to capture contextual information about retinal vessel configurations, leading to challenges in reconciling semantic disparities between encoder and decoder features. To address this, we propose a novel feature enhancement segmentation network (FES-Net) that achieves accurate pixel-wise segmentation without requiring additional image enhancement steps. FES-Net directly processes the input image and utilizes four prompt convolutional blocks (PCBs) during downsampling, complemented by a shallow upsampling approach to generate a binary mask for each class. We evaluate the performance of FES-Net on four publicly available state-of-the-art datasets: DRIVE, STARE, CHASE, and HRF. The evaluation results clearly demonstrate the superior performance of FES-Net compared to other competitive approaches documented in the existing literature.

==> References.tex <==
% Encoding: UTF-8

@article{tabassum2020cded,
  title={CDED-Net: Joint segmentation of optic disc and optic cup for glaucoma screening},
  author={Tabassum, Munazza and Khan, Tariq M and Arsalan, Muhammad and Naqvi, Syed Saud and Ahmed, Mansoor and Madni, Hussain Ahmed and Mirza, Jawad},
  journal={IEEE Access},
  volume={8},
  pages={102733--102747},
  year={2020},
  publisher={IEEE}
}

@article{abdullah2021review,
  title={A review on glaucoma disease detection using computerized techniques},
  author={Abdullah, Faizan and Imtiaz, Rakhshanda and Madni, Hussain Ahmad and Khan, Haroon Ahmed and Khan, Tariq M and Khan, Mohammad AU and Naqvi, Syed Saud},
  journal={IEEE Access},
  volume={9},
  pages={37311--37333},
  year={2021},
  publisher={IEEE}
}

@article{imtiaz2021screening,
  title={Screening of Glaucoma disease from retinal vessel images using semantic segmentation},
  author={Imtiaz, Rakhshanda and Khan, Tariq M and Naqvi, Syed Saud and Arsalan, Muhammad and Nawaz, Syed Junaid},
  journal={Computers \& Electrical Engineering},
  volume={91},
  pages={107036},
  year={2021},
  publisher={Elsevier}
}
@inproceedings{starkweather1991comparison,
  title={A Comparison of Genetic Sequencing Operators.},
  author={Starkweather, Timothy and McDaniel, S and Mathias, Keith E and Whitley, L Darrell and Whitley, C},
  booktitle={ICGA},
  pages={69--76},
  year={1991}
}
@InProceedings{Khan_2022_WACV,
    author    = {Khan, Tariq M. and Robles-Kelly, Antonio and Naqvi, Syed S.},
    title     = {T-Net: A Resource-Constrained Tiny Convolutional Neural Network for Medical Image Segmentation},
    booktitle = {Proceedings of the IEEE/CVF Winter Conference on Applications of Computer Vision (WACV)},
    month     = {January},
    year      = {2022},
    pages     = {644-653}
}

@article{KHAN2022103169,
title = {Width-wise vessel bifurcation for improved retinal vessel segmentation},
journal = {Biomedical Signal Processing and Control},
volume = {71},
pages = {103169},
year = {2022},
issn = {1746-8094},
doi = {https://doi.org/10.1016/j.bspc.2021.103169},
url = {https://www.sciencedirect.com/science/article/pii/S1746809421007667},
author = {Tariq M. Khan and Mohammad A.U. Khan and Naveed Ur Rehman and Khuram Naveed and Imran Uddin Afridi and Syed Saud Naqvi and Imran Raazak},
keywords = {Retinal vessels, Multiscale line detector, Diabetic retinopathy, Triple stick filter},
abstract = {Vessel local characteristics such as noise, illumination, and direction vary significantly in a fundus image, making it difficult to segment the vessel tree structure as a whole. To facilitate vessel detection, an alternative procedure proposed here, whereby retinal vessels first classified into two categories, large and small. Then, for its unique characteristics, each group has been processed with its own enhancement and detection filter. The sensitivity of the proposed method is boosted by capturing tiny vessels through a directional filter bank followed by its associated triple-stick filtering. Additionally, the specificity of the proposed method is enhanced through noise suppression attributed largely to the proposed BM3D filtering and multi-scale line detection approach. As a result, the detection accuracy on the DRIVE, STARE, and CHASE DB1 datasets is significantly improved, with scores of 0.9610, 0.9586, and 0.9578, respectively.}
}

@InProceedings{10.1007/978-3-030-73973-7_31,
author="Khan, Tariq M.
and Robles-Kelly, Antonio
and Naqvi, Syed S.
and Arsalan, Muhammad",
editor="Torsello, Andrea
and Rossi, Luca
and Pelillo, Marcello
and Biggio, Battista
and Robles-Kelly, Antonio",
title="Residual Multiscale Full Convolutional Network (RM-FCN) for High Resolution Semantic Segmentation of Retinal Vasculature",
booktitle="Structural, Syntactic, and Statistical Pattern Recognition",
year="2021",
publisher="Springer International Publishing",
address="Cham",
pages="324--333",
abstract="In a fundus image, Vessel local characteristics like direction, illumination and noise vary considerably, making vessel segmentation a challenging task. Methods based upon deep convolutional networks have consistently yield state of the art performance. Despite effective, of the drawbacks of these methods is their computational complexity, whereby testing and training of these networks require substantial computational resources and can be time consuming. Here we present a multi-scale kernel based on fully convolutional layers that is quite lightweight and can effectively segment large, medium, and thin vessels over a wide variations of contrast, position and size of the optic disk. Moreover, the architecture presented here makes use of these multi-scale kernels, reduced application of pooling operations and skip connections to achieve faster training. We illustrate the utility of our method for retinal vessel segmentation on the DRIVE, CHASE{\_}DB and STARE data sets. We also compare the results delivered by our method with a number of alternatives elsewhere in the literature. In our experiments, our method always provides a margin of improvement on specificity, accuracy, AUC and sensitivity with respect to the alternative.",
isbn="978-3-030-73973-7"
}
@article{khan2019generalized,
  title={A generalized multi-scale line-detection method to boost retinal vessel segmentation sensitivity},
  author={Khan, Mohammad AU and Khan, Tariq M and Bailey, Donald G and Soomro, Toufique A},
  journal={Pattern Analysis and Applications},
  volume={22},
  number={3},
  pages={1177--1196},
  year={2019},
  publisher={Springer London}
}

@article{khan2019ggm,
  title={Ggm classifier with multi-scale line detectors for retinal vessel segmentation},
  author={Khan, Mohammad AU and Khan, Tariq M and Naqvi, Syed S and Aurangzeb Khan, M},
  journal={Signal, Image and Video Processing},
  volume={13},
  number={8},
  pages={1667--1675},
  year={2019},
  publisher={Springer London}
}

@inproceedings{khan2019use,
  title={The use of fourier phase symmetry for thin vessel detection in retinal fundus images},
  author={Khan, Mohammad AU and Khan, Tariq M and Aziz, Kahtan I and Ahmad, Sayed S and Mir, Nighat and Elbakush, Emhemed},
  booktitle={2019 IEEE International Symposium on Signal Processing and Information Technology (ISSPIT)},
  pages={1--6},
  year={2019},
  organization={IEEE}
}

@article{khan2020residual,
  title={Residual connection-based encoder decoder network ({RCED-Net}) for retinal vessel segmentation},
  author={Khan, Tariq Mahmood and Alhussein, Musaed and Aurangzeb, Khursheed and Arsalan, Muhammad and Naqvi, Syed Saud and Nawaz, Syed Junaid},
  journal={IEEE Access},
  volume={8},
  pages={131257--131272},
  year={2020},
  publisher={IEEE}
}
@article{khan2020machine,
  title={Machine learning: Quantum vs classical},
  author={Khan, Tariq M and Robles-Kelly, Antonio},
  journal={IEEE Access},
  volume={8},
  pages={219275--219294},
  year={2020},
  publisher={IEEE}
}
@inproceedings{khan2020shallow,
  title={Shallow vessel segmentation network for automatic retinal vessel segmentation},
  author={Khan, Tariq M and Abdullah, Faizan and Naqvi, Syed S and Arsalan, Muhammad and Khan, Muhamamd Aurangzeb},
  booktitle={2020 International Joint Conference on Neural Networks (IJCNN)},
  pages={1--7},
  year={2020},
  organization={IEEE}
}

@inproceedings{khan2020exploiting,
  title={Exploiting residual edge information in deep fully convolutional neural networks for retinal vessel segmentation},
  author={Khan, Tariq M and Naqvi, Syed S and Arsalan, Muhammad and Khan, Muhamamd Aurangzeb and Khan, Haroon A and Haider, Adnan},
  booktitle={2020 International Joint Conference on Neural Networks (IJCNN)},
  pages={1--8},
  year={2020},
  organization={IEEE}
}

@inproceedings{khan2020semantically,
  title={A Semantically Flexible Feature Fusion Network for Retinal Vessel Segmentation},
  author={Khan, Tariq M and Robles-Kelly, Antonio and Naqvi, Syed S},
  booktitle={International Conference on Neural Information Processing},
  pages={159--167},
  year={2020},
  organization={Springer, Cham}
}

@inproceedings{khan2021rc,
  title={RC-Net: A Convolutional Neural Network for Retinal Vessel Segmentation},
  author={Khan, Tariq M and Robles--Kelly, Antonio and Naqvi, Syed S},
  booktitle={2021 Digital Image Computing: Techniques and Applications (DICTA)},
  pages={01--07},
  year={2021},
  organization={IEEE}
}

@ARTICLE{9422817,
  author={Zhou, Xiaokang and Xu, Xuesong and Liang, Wei and Zeng, Zhi and Yan, Zheng},
  journal={IEEE Internet of Things Journal}, 
  title={Deep-Learning-Enhanced Multitarget Detection for End–Edge–Cloud Surveillance in Smart IoT}, 
  year={2021},
  volume={8},
  number={16},
  pages={12588-12596},
  doi={10.1109/JIOT.2021.3077449}}


@ARTICLE{9093981,
  author={Zhou, Xiaokang and Li, Yue and Liang, Wei},
  journal={IEEE/ACM Transactions on Computational Biology and Bioinformatics}, 
  title={CNN-RNN Based Intelligent Recommendation for Online Medical Pre-Diagnosis Support}, 
  year={2021},
  volume={18},
  number={3},
  pages={912-921},
  doi={10.1109/TCBB.2020.2994780}}

@ARTICLE{8861193,
  author={Zhou, Xiaokang and Liang, Wei and Wang, Kevin I-Kai and Shimizu, Shohei},
  journal={IEEE Transactions on Computational Social Systems}, 
  title={Multi-Modality Behavioral Influence Analysis for Personalized Recommendations in Health Social Media Environment}, 
  year={2019},
  volume={6},
  number={5},
  pages={888-897},
  doi={10.1109/TCSS.2019.2918285}}


@ARTICLE{9090327,
  author={Zhou, Xiaokang and Liang, Wei and Wang, Kevin I-Kai and Yang, Laurence T.},
  journal={IEEE Transactions on Computational Social Systems}, 
  title={Deep Correlation Mining Based on Hierarchical Hybrid Networks for Heterogeneous Big Data Recommendations}, 
  year={2021},
  volume={8},
  number={1},
  pages={171-178},
  doi={10.1109/TCSS.2020.2987846}}


@ARTICLE{9363597,
  author={Zhou, Xiaokang and Xu, Xuesong and Liang, Wei and Zeng, Zhi and Shimizu, Shohei and Yang, Laurence T. and Jin, Qun},
  journal={IEEE Transactions on Industrial Informatics}, 
  title={Intelligent Small Object Detection for Digital Twin in Smart Manufacturing With Industrial Cyber-Physical Systems}, 
  year={2022},
  volume={18},
  number={2},
  pages={1377-1386},
  doi={10.1109/TII.2021.3061419}}


@Article{You2012a,
  author   = {Xinge You and Qinmu Peng and Yuan Yuan and Yiu-ming Cheung and Jiajia Lei},
  journal  = {Pattern Recognition},
  title    = {Segmentation of retinal blood vessels using the radial projection and semi-supervised approach},
  year     = {2012a},
  issn     = {0031-3203},
  note     = {Semi-Supervised Learning for Visual Content Analysis and Understanding},
  number   = {10},
  pages    = {2314 - 2324},
  volume   = {44},
  abstract = {Automatic segmentation of retinal blood vessels has become a necessary diagnostic procedure in ophthalmology. The blood vessels consist of two types of vessels, i.e., thin vessels and wide vessels. Therefore, a segmentation method may require two different processes to treat different vessels. However, traditional segmentation algorithms hardly draw a distinction between thin and wide vessels, but deal with them together. The major problems of these methods are as follows: (1) If more emphasis is placed on the extraction of thin vessels, the wide vessels tend to be over detected; and more artificial vessels are generated, too. (2) If more attention is paid on the wide vessels, the thin and low contrast vessels are likely to be missing. To overcome these problems, a novel scheme of extracting the retinal vessels based on the radial projection and semi-supervised method is presented in this paper. The radial projection method is used to locate the vessel centerlines which include the low-contrast and narrow vessels. Further, we modify the steerable complex wavelet to provide better capability of enhancing vessels under different scales, and construct the vector feature to represent the vessel pixel by line strength. Then, semi-supervised self-training is used for extraction of the major structures of vessels. The final segmentation is obtained by the union of the two types of vessels. Our approach is tested on two publicly available databases. Experiment results show that the method can achieve improved detection of thin vessels and decrease false detection of vessels in pathological regions compared to rival solutions.},
  doi      = {https://doi.org/10.1016/j.patcog.2011.01.007},
  keywords = {Radial projection, Retinal images, Steerable complex wavelet},
}

@Article{Abramoff2013,
  author  = {Abramoff, Michael and Folk, James and Han, Dennis and Walker, Jonathan and Williams, David and Russell, Stephen and Massin, Pascale and Cochener, Beatrice and Gain, Philippe and Tang, Li and Lamard, Mathieu and Moga, Daniela and Quellec, Gwenole and Niemeijer, Meindert},
  journal = {JAMA ophthalmology},
  title   = {Automated analysis of retinal images for detection of referable diabetic retinopathy},
  year    = {2013},
  month   = {03},
  pages   = {351-357},
  volume  = {131},
  doi     = {10.1001/jamaophthalmol.2013.1743},
}

@Article{Zeng2019,
  author  = {X. {Zeng} and H. {Chen} and Y. {Luo} and W. {Ye}},
  journal = {IEEE Access},
  title   = {Automated Diabetic Retinopathy Detection Based on Binocular Siamese-Like Convolutional Neural Network},
  year    = {2019},
  pages   = {30744-30753},
  volume  = {7},
}

@Article{Gao2019,
  author  = {Z. {Gao} and J. {Li} and J. {Guo} and Y. {Chen} and Z. {Yi} and J. {Zhong}},
  journal = {IEEE Access},
  title   = {Diagnosis of Diabetic Retinopathy Using Deep Neural Networks},
  year    = {2019},
  pages   = {3360-3370},
  volume  = {7},
}

@InProceedings{Thakoor2019,
  author    = {K. A. {Thakoor} and X. {Li} and E. {Tsamis} and P. {Sajda} and D. C. {Hood}},
  booktitle = {2019 41st Annual International Conference of the IEEE Engineering in Medicine and Biology Society (EMBC)},
  title     = {Enhancing the Accuracy of Glaucoma Detection from OCT Probability Maps using Convolutional Neural Networks},
  year      = {2019},
  pages     = {2036-2040},
  file      = {:Thakoor2019 - Enhancing the Accuracy of Glaucoma Detection from OCT Probability Maps Using Convolutional Neural Networks.ris:ris},
}

@Article{Cicinelli2018,
  author   = {Maria Vittoria Cicinelli and Alessandro Rabiolo and Riccardo Sacconi and Adriano Carnevali and Lea Querques and Francesco Bandello and Giuseppe Querques},
  journal  = {Survey of Ophthalmology},
  title    = {Optical coherence tomography angiography in dry age-related macular degeneration},
  year     = {2018},
  issn     = {0039-6257},
  number   = {2},
  pages    = {236-244},
  volume   = {63},
  abstract = {Optical coherence tomography angiography is a new imaging modality that provides noninvasive characterization and quantification of the microvasculature in different retinal conditions. The purpose of this study was to give an updated review of the features of dry age-related macular degeneration investigated by means of new-generation optical coherence tomography angiography. We searched PubMed and Medline using the terms “optical coherence tomography angiography” associated with “age-related macular degeneration,” “drusen,” “reticular pseudodrusen,” and “geographic atrophy” and reviewed publications up to January 2017.},
  doi      = {https://doi.org/10.1016/j.survophthal.2017.06.005},
  file     = {:S138650561831195X.ris:ris},
  keywords = {reticular pseudodrusen, drusen, age-related macular degeneration, geographic atrophy, optical coherence tomography angiography},
}

@Article{Muraoka2013,
  author  = {Yuki Muraoka and Akitaka Tsujikawa and Tomoaki Murakami and Ken Ogino and Kyoko Kumagai and Kazuaki Miyamoto and Akihito Uji and Nagahisa Yoshimura},
  journal = {Ophthalmology},
  title   = {Morphologic and Functional Changes in Retinal Vessels Associated with Branch Retinal Vein Occlusion},
  year    = {2013},
  issn    = {0161-6420},
  number  = {1},
  pages   = {91 - 99},
  volume  = {120},
  file    = {:Muraoka2013 - Morphologic and Functional Changes in Retinal Vessels Associated with Branch Retinal Vein Occlusion.bib:bib;:Muraoka2013 - Morphologic and Functional Changes in Retinal Vessels Associated with Branch Retinal Vein Occlusion.ris:ris},
}

@Article{Traustason2011,
  author  = {S. Traustason and A. S. Jensen and H. S. Arvidsson and I. C. Munch and L. Søndergaard and M. Larsen},
  journal = {Investigative Ophthalmology \& Visual Science},
  title   = {Retinal Oxygen Saturation in Patients with Systemic Hypoxemia},
  year    = {2011},
  number  = {8},
  pages   = {5064},
  volume  = {52},
}

@Article{Soomro2018,
  author      = {Soomro, T. A. and Khan, T. Mahmood and Khan, M. A. U. and Gao, J. and Paul, M. and Zheng, L.},
  journal     = {IEEE Access},
  title       = {Impact of {ICA}-Based Image Enhancement Technique on Retinal Blood Vessels Segmentation},
  year        = {2018},
  issn        = {2169-3536},
  pages       = {3524--3538},
  volume      = {6},
  call-number = {6},
  keywords    = {blood vessels, diseases, eye, image colour analysis, image enhancement, image segmentation, independent component analysis, medical image processing, retinal blood vessels segmentation, automatic retinal vessel segmentation method, eye vessels, eye diseases, retinal color fundus images, ICA2 architecture, ICA-based image enhancement technique, independent component analysis, DRIVE database, STARE database, Retina, Image segmentation, Biomedical imaging, Blood vessels, Image color analysis, Diseases, Independent component analysis, Retinal, segmentation, morphological filtering, ICA vessel enhancement},
}

@Article{Singh2018,
  author   = {Singh, S R and Handa, S and Dogra, M and Dogra, M R},
  journal  = {QJM: An International Journal of Medicine},
  title    = {{Fundoscopy and malignant hypertension}},
  year     = {2018},
  issn     = {1460-2725},
  month    = {11},
  number   = {4},
  pages    = {305-305},
  volume   = {112},
}

@Article{Narayanan2015,
  author  = {Narayanan, Anuradha and Ramani, Krishnakumar},
  journal = {Oman journal of ophthalmology},
  title   = {Role of optometry school in single day large scale school vision testing},
  year    = {2015},
  month   = {02},
  pages   = {28-32},
  volume  = {8},
  doi     = {10.4103/0974-620X.149861},
  file    = {:Narayanan2015 - Role of Optometry School in Single Day Large Scale School Vision Testing.ris:ris},
}

@Article{Kirbas2004,
  author  = {C. Kirbas and F. Quek},
  journal = {ACM Comput. Surv.},
  title   = {A Review of Vessel Extraction Techniques and Algorithms},
  year    = {2004},
  number  = {2},
  pages   = {81--121},
  volume  = {36},
}

@Article{Jiang2019,
  author  = {Y. {Jiang} and N. {Tan} and T. {Peng}},
  journal = {IEEE Access},
  title   = {Optic Disc and Cup Segmentation Based on Deep Convolutional Generative Adversarial Networks},
  year    = {2019},
  pages   = {64483-64493},
  volume  = {7},
}

@Article{Yu2019,
  author   = {Shuang Yu and Di Xiao and Shaun Frost and Yogesan Kanagasingam},
  journal  = {Computerized Medical Imaging and Graphics},
  title    = {Robust optic disc and cup segmentation with deep learning for glaucoma detection},
  year     = {2019},
  issn     = {0895-6111},
  pages    = {61 - 71},
  volume   = {74},
  }

@Article{Jiang2019a,
  author  = {Jiang, Yun and Zhang, Hai and Tan, Ning and Chen, Li},
  journal = {Symmetry},
  title   = {Automatic Retinal Blood Vessel Segmentation Based on Fully Convolutional Neural Networks},
  year    = {2019},
  month   = {09},
  pages   = {1112},
  volume  = {11},
  doi     = {10.3390/sym11091112},
}

@InProceedings{Li2018,
  author = {Li, Ming and Yin, Qingbo and Lu, Mingyu},
  title  = {Retinal Blood Vessel Segmentation Based on Multi-Scale Deep Learning},
  year   = {2018},
  month  = {09},
  pages  = {117-123},
  doi    = {10.15439/2018F127},
}

@Article{Badrinarayanan2017,
  author  = {V. Badrinarayanan and A. Kendall and R. Cipolla},
  journal = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
  title   = {{SegNet}: A Deep Convolutional Encoder-Decoder Architecture for Image Segmentation},
  year    = {2017},
  number  = {12},
  pages   = {2481-2495},
  volume  = {39},
}

@Article{Zhao2015,
  author  = {Y. {Zhao} and L. {Rada} and K. {Chen} and S. P. {Harding} and Y. {Zheng}},
  journal = {IEEE Transactions on Medical Imaging},
  title   = {Automated Vessel Segmentation Using Infinite Perimeter Active Contour Model with Hybrid Region Information with Application to Retinal Images},
  year    = {2015},
  number  = {9},
  pages   = {1797-1807},
  volume  = {34},
}

@Article{Jin2019,
  author   = {Qiangguo Jin and Zhaopeng Meng and Tuan D. Pham and Qi Chen and Leyi Wei and Ran Su},
  journal  = {Knowledge-Based Systems},
  title    = {{DUNet}: A deformable network for retinal vessel segmentation},
  year     = {2019},
  issn     = {0950-7051},
  pages    = {149-162},
  volume   = {178},
}

@Article{Zhang2014,
  author   = {Jia Zhang and Huiqi Li and Qing Nie and Li Cheng},
  journal  = {Computerized Medical Imaging and Graphics},
  title    = {A retinal vessel boundary tracking method based on Bayesian theory and multi-scale line detection},
  year     = {2014},
  issn     = {0895-6111},
  number   = {6},
  pages    = {517 - 525},
  volume   = {38},
}

@Article{Gang2002,
  author  = {L. Gang and O. Chutatape and S. M. Krishnan},
  journal = {IEEE Transactions on Biomedical Engineering},
  title   = {Detection and measurement of retinal vessels in fundus images using amplitude modified second-order Gaussian filter},
  year    = {2002},
  number  = {2},
  pages   = {168-172},
  volume  = {49},
}

@Article{Lam2008,
  author  = {B. S. Y. Lam and H. Yan},
  journal = {IEEE Transactions on Medical Imaging},
  title   = {{A novel vessel segmentation algorithm for pathological retina images based on the divergence of vector fields}},
  year    = {2008},
  number  = {2},
  pages   = {237--246},
  volume  = {27},
}

@InProceedings{Espona2008,
  author    = {L. Espona and M. J. Carreira and M. G. Penedo and M. Ortega},
  booktitle = {2008 19th International Conference on Pattern Recognition},
  title     = {Retinal vessel tree segmentation using a deformable contour model},
  year      = {2008},
  pages     = {1-4},
}

@Article{Sum2008,
  author  = {K. W. Sum and P. Y. S. Cheung},
  journal = {IEEE Transactions on Biomedical Engineering},
  title   = {Vessel Extraction Under Non-Uniform Illumination: A Level Set Approach},
  year    = {2008},
  number  = {1},
  pages   = {358-360},
  volume  = {55},
}

@Article{Soares2006,
  author  = {J. V. B. Soares and J. J. G. Leandro and R. M. Cesar and H. F. Jelinek and M. J. Cree},
  journal = {IEEE Transactions on Medical Imaging},
  title   = {Retinal vessel segmentation using the 2-D Gabor wavelet and supervised classification},
  year    = {2006},
  number  = {9},
  pages   = {1214-1222},
  volume  = {25},
}

@Article{Memari2017,
  author    = {Memari, Nogol AND Ramli, Abd Rahman AND Bin Saripan, M. Iqbal AND Mashohor, Syamsiah AND Moghbel, Mehrdad},
  journal   = {PLOS ONE},
  title     = {Supervised retinal vessel segmentation from color fundus images based on matched filtering and AdaBoost classifier},
  year      = {2017},
  month     = {12},
  number    = {12},
  pages     = {1-35},
  volume    = {12},
}

@Article{Roychowdhury2015,
  author  = {S. Roychowdhury and D. D. Koozekanani and K. K. Parhi},
  journal = {IEEE Journal of Biomedical and Health Informatics},
  title   = {Blood Vessel Segmentation of Fundus Images by Major Vessel Extraction and Subimage Classification},
  year    = {2015},
  number  = {3},
  pages   = {1118-1128},
  volume  = {19},
}

@Article{Colomer2020,
  author         = {Colomer, Adrián and Igual, Jorge and Naranjo, Valery},
  journal        = {Sensors},
  title          = {Detection of Early Signs of Diabetic Retinopathy Based on Textural and Morphological Information in Fundus Images},
  year           = {2020},
  issn           = {1424-8220},
  number         = {4},
  volume         = {20},
}

@Article{Staal2004,
  author  = {J. Staal and M. D. Abramoff and M. Niemeijer and M. A. Viergever and B. van Ginneken},
  journal = {IEEE Transactions on Medical Imaging},
  title   = {Ridge-based vessel segmentation in color images of the retina},
  year    = {2004},
  number  = {4},
  pages   = {501-509},
  volume  = {23},
}

@Article{Ricci2007,
  author  = {E. Ricci and R. Perfetti},
  journal = {IEEE Transactions on Medical Imaging},
  title   = {Retinal Blood Vessel Segmentation Using Line Operators and Support Vector Classification},
  year    = {2007},
  number  = {10},
  pages   = {1357-1365},
  volume  = {26},
}

@Article{Jiang2019b,
  author  = {Y. Jiang and N. Tan and T.Peng and H. Zhang},
  journal = {IEEE Access},
  title   = {Retinal Vessels Segmentation Based on Dilated Multi-Scale Convolutional Neural Network},
  year    = {2019},
  pages   = {76342-76352},
  volume  = {7},
}

@Article{Soomro2019,
  author   = {Toufique Ahmed Soomro and Ahmed J. Afifi and Junbin Gao and Olaf Hellwich and Lihong Zheng and Manoranjan Paul},
  journal  = {Expert Systems with Applications},
  title    = {Strided fully convolutional neural network for boosting the sensitivity of retinal blood vessels segmentation},
  year     = {2019},
  issn     = {0957-4174},
  pages    = {36-52},
  volume   = {134},
}

@InProceedings{Ladicky2010,
  author    = {Ladick{\'y}, L. and Sturgess, P. and Alahari, K. and Russell, C. and Torr, P. H. S.},
  booktitle = {Computer Vision -- ECCV 2010},
  title     = {What, Where and How Many? Combining Object Detectors and CRFs},
  year      = {2010},
  address   = {Berlin, Heidelberg},
  editor    = {Daniilidis, Kostas and Maragos, Petros and Paragios, Nikos},
  pages     = {424--437},
  publisher = {Springer Berlin Heidelberg},
  abstract  = {Computer vision algorithms for individual tasks such as object recognition, detection and segmentation have shown impressive results in the recent past. The next challenge is to integrate all these algorithms and address the problem of scene understanding. This paper is a step towards this goal. We present a probabilistic framework for reasoning about regions, objects, and their attributes such as object class, location, and spatial extent. Our model is a Conditional Random Field defined on pixels, segments and objects. We define a global energy function for the model, which combines results from sliding window detectors, and low-level pixel-based unary and pairwise relations. One of our primary contributions is to show that this energy function can be solved efficiently. Experimental results show that our model achieves significant improvement over the baseline methods on CamVid and pascal voc datasets.},
  file      = {:Ladicky2010 - What, Where and How Many_ Combining Object Detectors and CRFs.bib:bib},
  isbn      = {978-3-642-15561-1},
}

@Article{Zhang2016,
  author      = {J. Zhang and B. Dashtbozorg and E. Bekkers and J. P. W. Pluim and R. Duits and B. M. Romeny},
  journal     = {IEEE Transactions on Medical Imaging},
  title       = {Robust Retinal Vessel Segmentation via Locally Adaptive Derivative Frames in Orientation Scores},
  year        = {2016},
  issn        = {0278-0062},
  number      = {12},
  pages       = {2631--2644},
  volume      = {35},
  call-number = {35},
  file        = {:Zhang2016 - Robust Retinal Vessel Segmentation Via Locally Adaptive Derivative Frames in Orientation Scores.ris:ris},
  keywords    = {biomedical optical imaging, blood vessels, diseases, eye, Gaussian processes, image segmentation, Lie groups, medical image processing, reviews, vision defects, LAD filter, LAD filter on orientation scores, (LAD-OS), state-of-the-art methods, central arterial reflex, retinal image datasets, binary segmentation, enhanced vessels, 2D image plane, orientation score domain, multi-scale filtering, left-invariant Hessian matrix, eigensystem analysis, local line structures, (LAD) frame, locally adaptive derivative frame, left-invariant rotating derivative frame, line structures, multi-scale second-order Gaussian derivatives, orientation planes, elongated structures, 3D orientation score, 2D image, wavelet-type transform, Lie-group domain, 3D rotating frames, robust-fully automatic filter-based approach, locally adaptive derivative frames, robust retinal vessel segmentation, Image segmentation, Retinal vessels, Robustness, Transforms, Two dimensional displays, Feature extraction, Gaussian derivatives, orientation scores, retinal image analysis, rotating filter, vessel segmentation, Algorithms, Databases, Factual, Humans, Image Interpretation, Computer-Assisted, Image Processing, Computer-Assisted, Ophthalmoscopy, Retinal Vessels, Wavelet Analysis},
}

@Article{Zhang2010,
  author   = {Zhang, B. and Zhang, L. and Zhang, L. and Karray, F.},
  journal  = {Computers in Biology and Medicine},
  title    = {Retinal vessel extraction by matched filter with first-order derivative of Gaussian},
  year     = {2010},
  issn     = {0010-4825},
  month    = apr,
  number   = {4},
  pages    = {438--445},
  volume   = {40},
}

@Article{Lam2010,
  author      = {B. S. Y. Lam and Y. Gao and A. W. Liew},
  journal     = {IEEE Transactions on Medical Imaging},
  title       = {General Retinal Vessel Segmentation Using Regularization-Based Multiconcavity Modeling},
  year        = {2010},
  issn        = {0278-0062},
  number      = {7},
  pages       = {1369--1381},
  volume      = {29},
  call-number = {29},
  keywords    = {biomedical optical imaging, blood vessels, eye, image denoising, image segmentation, medical image processing, retinal vessel segmentation, regularization based multiconcavity modeling, blood vessel detection, retinal images, bright lesions, dark lesions, differentiable concavity measure, perceptive space, line shape concavity measure, lesion intensity structure, line shaped vessels, unevenly distributed noise, retinal image spherical intensity variation, Retinal vessels, Retina, Lesions, Image segmentation, Blood vessels, Biomedical imaging, Extraterrestrial measurements, Noise measurement, Statistical distributions, Humans, Multiconcavity modeling, perceptive transform, regularization, retina image, retinal vessel segmentation, Algorithms, Computer Simulation, Humans, Image Enhancement, Image Interpretation, Computer-Assisted, Information Storage and Retrieval, Models, Biological, Pattern Recognition, Automated, Reproducibility of Results, Retinal Vessels, Retinoscopy, Sensitivity and Specificity},
}

@Article{Miri2011,
  author      = {Miri, M. S. and Mahloojifar, A.},
  journal     = {IEEE Transactions on Biomedical Engineering},
  title       = {Retinal Image Analysis Using Curvelet Transform and Multistructure Elements Morphology by Reconstruction},
  year        = {2011},
  issn        = {0018-9294},
  number      = {5},
  pages       = {1183--1192},
  volume      = {58},
  call-number = {58},
  keywords    = {biomedical optical imaging, blood vessels, curvelet transforms, eye, image reconstruction, image segmentation, medical image processing, patient diagnosis, retinal image analysis, curvelet transform, image reconstruction, ocular fundus operations, human recognition, early stage disease detection, diabetes, retinal blood vessels, image segmentation, multistructure elements method, morphology operators, connected components analysis, DRIVE, blood vessel detection, Image edge detection, Retina, Transforms, Image reconstruction, Morphology, Blood vessels, Biomedical imaging, Blood vessel segmentation, curvelet transform, morphology operators by reconstruction, multistructure elements morphology, retinal image, Algorithms, Databases, Factual, Diagnostic Techniques, Ophthalmological, Fundus Oculi, Humans, Image Processing, Computer-Assisted, Models, Statistical, Retinal Vessels},
}

@Article{Fraz2012c,
  author   = {M. M. Fraz and S.A. Barman and P. Remagnino and A. Hoppe and A. Basit and B. Uyyanonvara and A. R. Rudnicka and C. G. Owen},
  journal  = {Computer Methods and Programs in Biomedicine},
  title    = {An approach to localize the retinal blood vessels using bit planes and centerline detection},
  year     = {2012c},
  issn     = {0169-2607},
  number   = {2},
  pages    = {600 - 616},
  volume   = {108},
}

@Article{Azzopardi2015,
  author   = {G. Azzopardi and N. Strisciuglio and M. Vento and N. Petkov},
  journal  = {Medical Image Analysis},
  title    = {{Trainable COSFIRE filters for vessel delineation with application to retinal images}},
  year     = {2015},
  number   = {1},
  pages    = {46--57},
  volume   = {19},
  keywords = {COSFIRE,Delineation,Retinal image analysis,Trainable filters,Vessel segmentation},
}

@Article{Yin2015,
  author   = {B. Yin and H. Li and B. Sheng and X. Hou and Y. Chen and W. Wu and P. Li and R. Shen and Y. Bao and W. Jia},
  journal  = {Medical Image Analysis},
  title    = {Vessel extraction from non-fluorescein fundus images using orientation-aware detector},
  year     = {2015},
  issn     = {1361-8415},
  number   = {1},
  pages    = {232 - 242},
  volume   = {26},
}

@Article{Fraz2011,
  author  = {M. M. Fraz and P. Remagnino abd A. Hoppe and B. Uyyanonvara and A. R. Rudnicka and C. G. Owen and S. A. Barman},
  journal = {Computer Methods and Programs in Biomedicine},
  title   = {Blood vessel segmentation methodologies in retinal images – A survey},
  year    = {2011},
  number  = {1},
  pages   = {407 - 433},
  volume  = {108},
}

@Article{Cheng2014,
  author  = {E. Cheng and L. Du and Y. Wu and Y. J. Zhu and V. Megalooikonomou and H. Ling},
  journal = {Machine Vision and Applications},
  title   = {Discriminative vessel segmentation in retinal images by fusing context-aware hybrid features},
  year    = {2014},
  issn    = {1432-1769},
  month   = oct,
  number  = {7},
  pages   = {1779--1792},
  volume  = {25},
  refid   = {Cheng2014},
}

@Article{Li2016,
  author  = {Q. Li and B. Feng and L. Xie and P. Liang and H. Zhang and T. Wang},
  journal = {IEEE Transactions on Medical Imaging},
  title   = {A Cross-Modality Learning Approach for Vessel Segmentation in Retinal Images},
  year    = {2016},
  number  = {1},
  pages   = {109-118},
  volume  = {35},
}

@Article{Orlando2016,
  author      = {Orlando, J. I. and Prokofyeva, E. and Blaschko, M. B.},
  journal     = {IEEE Transactions on Biomedical Engineering},
  title       = {A Discriminatively Trained Fully Connected Conditional Random Field Model for Blood Vessel Segmentation in Fundus Images},
  year        = {2016},
  issn        = {0018-9294},
  number      = {1},
  pages       = {16--27},
  volume      = {64},
  call-number = {64},
  keywords    = {biomedical optical imaging, blood vessels, eye, image segmentation, medical image processing, support vector machines, elongated structure segmention, local neighborhood-based approach, HRF dataset, CHASEDB1 dataset, STARE dataset, DRIVE dataset, machine learning application, support vector machine, conditional random field model, fundus image, blood vessel segmentation, Image segmentation, Biomedical imaging, Blood vessels, Support vector machines, Retina, Standards, Diseases, Blood vessel segmentation, conditional random fields (CRFs), fundus imaging, structured output support vector machine (SOSVM), Computer Simulation, Fluorescein Angiography, Humans, Image Interpretation, Computer-Assisted, Machine Learning, Models, Cardiovascular, Models, Statistical, Ophthalmoscopy, Pattern Recognition, Automated, Photography, Reproducibility of Results, Retinal Artery, Retinal Diseases, Sensitivity and Specificity},
}

@InProceedings{Dasgupta2017,
  author    = {Dasgupta, A. and Singh, S.},
  booktitle = {IEEE 14th International Symposium on Biomedical Imaging (ISBI 2017)},
  title     = {A fully convolutional neural network based structured prediction approach towards the retinal vessel segmentation},
  year      = {2017},
  pages     = {248--251},
  file      = {:Dasgupta2017 - A Fully Convolutional Neural Network Based Structured Prediction Approach Towards the Retinal Vessel Segmentation.ris:ris},
  issn      = {1945-8452},
  journal   = {2017 IEEE 14th International Symposium on Biomedical Imaging (ISBI 2017)},
  keywords  = {blood vessels, eye, image segmentation, medical image processing, neural nets, fully convolutional neural network, retinal vessel segmentation, multilabel inference task, automatic retinal blood vessel segmentation, Image segmentation, Biomedical imaging, Blood vessels, Neural networks, Retinal vessels, Feature extraction, Computer-aided diagnosis, retinal vessels, convolution neural networks, image segmentation},
}

@Article{Marin2011,
  author  = {D. Marin and A. Aquino and M. E. Gegundez-Arias and J. M. Bravo},
  journal = {IEEE Transactions on Medical Imaging},
  title   = {A New Supervised Method for Blood Vessel Segmentation in Retinal Images by Using Gray-Level and Moment Invariants-Based Features},
  year    = {2011},
  number  = {1},
  pages   = {146-158},
  volume  = {30},
}

@Article{Shin2019,
  author   = {Seung Yeon Shin and Soochahn Lee and Il Dong Yun and Kyoung Mu Lee},
  journal  = {Medical Image Analysis},
  title    = {Deep vessel segmentation by learning graphical connectivity},
  year     = {2019},
  issn     = {1361-8415},
  pages    = {101556},
  volume   = {58},
}

@Article{Adapa2020,
  author    = {Adapa, Dharmateja AND Joseph Raj, Alex Noel AND Alisetti, Sai Nikhil AND Zhuang, Zhemin AND K., Ganesan AND Naik, Ganesh},
  journal   = {PLOS ONE},
  title     = {A supervised blood vessel segmentation technique for digital Fundus images using Zernike Moment based features},
  year      = {2020},
  month     = {03},
  number    = {3},
  pages     = {1-23},
  volume    = {15},
}

@Article{Jiang2019c,
  author  = {Y. {Jiang} and N. {Tan} and T. {Peng} and H. {Zhang}},
  journal = {IEEE Access},
  title   = {Retinal Vessels Segmentation Based on Dilated Multi-Scale Convolutional Neural Network},
  year    = {2019},
  pages   = {76342-76352},
  volume  = {7},
}

@Article{You2011,
  author   = {Xinge You and Qinmu Peng and Yuan Yuan and Yiu-ming Cheung and Jiajia Lei},
  journal  = {Pattern Recognition},
  title    = {Segmentation of retinal blood vessels using the radial projection and semi-supervised approach},
  year     = {2011},
  issn     = {0031-3203},
  note     = {Semi-Supervised Learning for Visual Content Analysis and Understanding},
  number   = {10},
  pages    = {2314 - 2324},
  volume   = {44},
}

@Article{Roychowdhury2014,
  author  = {Roychowdhury, Sohini and Koozekanani, Dara and Parhi, Keshab},
  journal = {IEEE journal of biomedical and health informatics},
  title   = {Blood Vessel Segmentation of Fundus Images by Major Vessel Extraction and Sub-Image Classification},
  year    = {2014},
  month   = {07},
  volume  = {19},
  doi     = {10.1109/JBHI.2014.2335617},
}

@InProceedings{Brostow2008,
  author    = {Brostow, G. J. and Shotton, J. and Fauqueur, J. and Cipolla, R.},
  booktitle = {Computer Vision -- ECCV 2008},
  title     = {Segmentation and Recognition Using Structure from Motion Point Clouds},
  year      = {2008},
  address   = {Berlin, Heidelberg},
  editor    = {Forsyth, David and Torr, Philip and Zisserman, Andrew},
  pages     = {44--57},
  publisher = {Springer Berlin Heidelberg},
  abstract  = {We propose an algorithm for semantic segmentation based on 3D point clouds derived from ego-motion. We motivate five simple cues designed to model specific patterns of motion and 3D world structure that vary with object category. We introduce features that project the 3D cues back to the 2D image plane while modeling spatial layout and context. A randomized decision forest combines many such features to achieve a coherent 2D segmentation and recognize the object categories present. Our main contribution is to show how semantic segmentation is possible based solely on motion-derived 3D world structure. Our method works well on sparse, noisy point clouds, and unlike existing approaches, does not need appearance-based descriptors.},
  isbn      = {978-3-540-88682-2},
}

@Article{Shelhamer2017,
  author      = {Shelhamer, E. and Long, J. and Darrell, T.},
  journal     = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
  title       = {Fully Convolutional Networks for Semantic Segmentation},
  year        = {2017},
  issn        = {0162-8828},
  number      = {4},
  pages       = {640--651},
  volume      = {39},
  call-number = {39},
  file        = {:Shelhamer2017 - Fully Convolutional Networks for Semantic Segmentation.bib:bib},
  keywords    = {feedforward neural nets, image classification, image representation, image resolution, image segmentation, learning (artificial intelligence), transforms, fully convolutional networks, semantic segmentation, visual models, correspondingly-sized output, spatially dense prediction tasks, contemporary classification networks, learned representations, coarse layer, fine layer, PASCAL VOC, NYUDv2, SIFT Flow, PASCAL-Context, Semantics, Image segmentation, Training, Convolution, Computer architecture, Proposals, Fuses, Semantic Segmentation, Convolutional Networks, Deep Learning, Transfer Learning},
}

@InCollection{Ciresan2012,
  author    = {D. Ciresan and A. Giusti and L. M. Gambardella and Schmidhuber, J\"{u}rgen},
  booktitle = {Advances in Neural Information Processing Systems 25},
  publisher = {Curran Associates, Inc.},
  title     = {Deep Neural Networks Segment Neuronal Membranes in Electron Microscopy Images},
  year      = {2012},
  editor    = {F. Pereira and C. J. C. Burges and L. Bottou and K. Q. Weinberger},
  pages     = {2843--2851},
}

@Article{Farabet2013,
  author      = {Farabet, C. and Couprie, C. and Najman, L. and LeCun, Y.},
  journal     = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
  title       = {Learning Hierarchical Features for Scene Labeling},
  year        = {2013},
  issn        = {0162-8828},
  number      = {8},
  pages       = {1915--1929},
  volume      = {35},
  call-number = {35},
  keywords    = {feature extraction, image classification, image segmentation, image texture, shape recognition, transforms, trees (mathematics), hierarchical feature learning, scene labeling, image pixel labeling, object category, multiscale convolutional network, dense feature vector extraction, multiple size region encoding, contextual information capturing, shape information capturing, texture information capturing, segmentation components, segmentation tree, SIFT flow dataset, Barcelona dataset, near-record accuracy, Stanford background dataset, image labeling, Feature extraction, Image segmentation, Labeling, Vectors, Context, Image edge detection, Accuracy, Convolutional networks, deep learning, image segmentation, image classification, scene parsing},
}

@Article{Chen2014,
  author        = {L. Chen and G. Papandreou and I. Kokkinos and K. Murphy and A. L. Yuille},
  journal       = {CoRR},
  title         = {Semantic Image Segmentation with Deep Convolutional Nets and Fully Connected CRFs},
  year          = {2014},
  volume        = {abs/1412.7062},
  archiveprefix = {arXiv},
  bibsource     = {dblp computer science bibliography, https://dblp.org},
  biburl        = {https://dblp.org/rec/bib/journals/corr/ChenPKMY14},
  eprint        = {1412.7062},
  timestamp     = {Mon, 13 Aug 2018 16:46:27 +0200},
}

@Article{Jiang2003,
  author      = {X. Jiang and D. Mojon},
  journal     = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
  title       = {Adaptive local thresholding by verification-based multithreshold probing with application to vessel detection in retinal images},
  year        = {2003},
  issn        = {0162-8828},
  number      = {1},
  pages       = {131--137},
  volume      = {25},
  call-number = {25},
  keywords    = {medical image processing, biometrics (access control), object detection, blood vessels, adaptive local thresholding, verification-based multithreshold probing, vessel detection, retinal images, object hypothesis generation, binarization, knowledge-guided adaptive thresholding, global thresholding, vessel detection method, Retina, Pixel, Application software, Histograms, Image segmentation, Biomedical imaging, Reflectivity, Lighting, Cameras, Shape},
}

@Article{Mendonca2006,
  author      = {A. M. Mendonca and A. Campilho},
  journal     = {IEEE Transactions on Medical Imaging},
  title       = {Segmentation of retinal blood vessels by combining the detection of centerlines and morphological reconstruction},
  year        = {2006},
  issn        = {0278-0062},
  number      = {9},
  pages       = {1200--1213},
  volume      = {25},
  call-number = {25},
  keywords    = {blood vessels, edge detection, eye, image reconstruction, image segmentation, iterative methods, medical image processing, retinal blood vessel segmentation, centerline detection, morphological reconstruction, vessel centerline extraction, directional differential operators, iterative region growing method, binary images, vessel width-dependent morphological filters, Retina, Blood vessels, Image segmentation, Biomedical imaging, Image reconstruction, Guidelines, Filling, Iterative methods, Filters, Testing, Edge detection, morphological processing, ophthalmology, retinal images, vessel segmentation, Algorithms, Artificial Intelligence, Humans, Image Enhancement, Image Interpretation, Computer-Assisted, Information Storage and Retrieval, Pattern Recognition, Automated, Reproducibility of Results, Retinal Vessels, Retinoscopy, Sensitivity and Specificity},
}

@Article{AlDiri2009,
  author      = {B. Al-Diri and A. Hunter and D. Steel},
  journal     = {IEEE Transactions on Medical Imaging},
  title       = {An Active Contour Model for Segmenting and Measuring Retinal Vessels},
  year        = {2009},
  issn        = {0278-0062},
  number      = {9},
  pages       = {1488--1497},
  volume      = {28},
  call-number = {28},
  keywords    = {blood vessels, eye, image segmentation, medical image processing, neural nets, retinal vessel segmentation, retinal vessel measurement, Ribbon of Twins active contour model, generalized morphological order filter, vessel centerline approximation, network topology, implicit neural cost function, junction configurations, Active contours, Retinal vessels, Electrostatic precipitators, Steel, Robustness, Measurement errors, Informatics, Shape measurement, Filters, Network topology, Parametric active contour, retinal vessel segmentation, Algorithms, Databases, Factual, Humans, Image Processing, Computer-Assisted, Models, Theoretical, Retinal Vessels},
}

@Article{Hoover2000,
  author      = {A. D. Hoover and V. Kouznetsova and M. Goldbaum},
  journal     = {IEEE Transactions on Medical Imaging},
  title       = {Locating blood vessels in retinal images by piecewise threshold probing of a matched filter response},
  year        = {2000},
  issn        = {0278-0062},
  number      = {3},
  pages       = {203--210},
  volume      = {19},
  call-number = {19},
  file        = {:Hoover2000 - Locating Blood Vessels in Retinal Images by Piecewise Threshold Probing of a Matched Filter Response.bib:bib},
  keywords    = {blood vessels, eye, image segmentation, medical image processing, optical images, matched filters, blood vessels location, retinal images, piecewise threshold probing, matched filter response, operating characteristic, true positive rate, false positive detection rate, eye care specialists, patient screening, treatment evaluation, clinical study, global vessel features, local vessel features, vessel network segmentation, Blood vessels, Biomedical imaging, Retina, Matched filters, Image segmentation, Medical treatment, Labeling, Diabetes, Hypertension, Arteriosclerosis, Algorithms, Humans, Image Processing, Computer-Assisted, Magnetic Resonance Imaging, Reproducibility of Results, Retina, Retinal Diseases, Retinal Vessels},
}

@Article{Khawaja2019,
  author         = {Khawaja, Ahsan and Khan, Tariq M. and Khan, Mohammad A. U. and Nawaz, Syed Junaid},
  title          = {A Multi-Scale Directional Line Detector for Retinal Vessel Segmentation},
  journal        = {Sensors},
  year           = {2019},
  volume         = {19},
  number         = {22},
  issn           = {1424-8220},
  abstract       = {The assessment of transformations in the retinal vascular structure has a strong potential in indicating a wide range of underlying ocular pathologies. Correctly identifying the retinal vessel map is a crucial step in disease identification, severity progression assessment, and appropriate treatment. Marking the vessels manually by a human expert is a tedious and time-consuming task, thereby reinforcing the need for automated algorithms capable of quick segmentation of retinal features and any possible anomalies. Techniques based on unsupervised learning methods utilize vessel morphology to classify vessel pixels. This study proposes a directional multi-scale line detector technique for the segmentation of retinal vessels with the prime focus on the tiny vessels that are most difficult to segment out. Constructing a directional line-detector, and using it on images having only the features oriented along the detector&rsquo;s direction, significantly improves the detection accuracy of the algorithm. The finishing step involves a binarization operation, which is again directional in nature, helps in achieving further performance improvements in terms of key performance indicators. The proposed method is observed to obtain a sensitivity of 0.8043, 0.8011, and 0.7974 for the Digital Retinal Images for Vessel Extraction (DRIVE), STructured Analysis of the Retina (STARE), and Child Heart And health Study in England (CHASE_DB1) datasets, respectively. These results, along with other performance enhancements demonstrated by the conducted experimental evaluation, establish the validity and applicability of directional multi-scale line detectors as a competitive framework for retinal image segmentation.},
  article-number = {4949},
}

@Article{Khawaja2019a,
  author   = {A. {Khawaja} and T. M. {Khan} and K. {Naveed} and S. S. {Naqvi} and N. U. {Rehman} and S. {Junaid Nawaz}},
  title    = {An Improved Retinal Vessel Segmentation Framework Using {Frangi} Filter Coupled With the Probabilistic Patch Based Denoiser},
  journal  = {IEEE Access},
  year     = {2019},
  volume   = {7},
  pages    = {164344-164361},
  issn     = {2169-3536},
  doi      = {10.1109/ACCESS.2019.2953259},
  keywords = {image denoising;image enhancement;image filtering;image segmentation;probability;retinal recognition;linear recombination;modified Frangi filter;Contrast Limited Adaptive Histogram Equalization;Generalized Linear Model;improved retinal vessel segmentation framework;detection accuracy;vessel contrast;observed noise level;vessel segmentation strategies;contrast enhancement;preprocessing step;vessel detection;state-of-the-art Probabilistic Patch-Based denoiser;unsupervised retinal vessel segmentation strategy;PPB denoiser;amplified noise;Image denoising;image segmentation;modified Frangi filter;probabilistic patch-based denoiser;retinal vessels},
}


@Article{aguirre2018blood,
  author    = {Aguirre-Ramos, Hugo and Avina-Cervantes, Juan Gabriel and Cruz-Aceves, Ivan and Ruiz-Pinales, Jos{\'e} and Ledesma, Sergio},
  title     = {Blood vessel segmentation in retinal fundus images using Gabor filters, fractional derivatives, and Expectation Maximization},
  journal   = {Applied Mathematics and Computation},
  year      = {2018},
  volume    = {339},
  pages     = {568--587},
  publisher = {Elsevier},
}

@Article{chen2018encoder,
  author    = {Chen, Liang-Chieh and Zhu, Yukun and Papandreou, George and Schroff, Florian and Adam, Hartwig},
  title     = {Encoder-Decoder with Atrous Separable Convolution for Semantic Image Segmentation},
  journal   = {Lecture Notes in Computer Science},
  year      = {2018},
  pages     = {833–851},
  issn      = {1611-3349},
  isbn      = {9783030012342},
  publisher = {Springer International Publishing},
}

@Article{zhang2016robust,
  author    = {Zhang, Jiong and Dashtbozorg, Behdad and Bekkers, Erik and Pluim, Josien PW and Duits, Remco and ter Haar Romeny, Bart M},
  title     = {Robust retinal vessel segmentation via locally adaptive derivative frames in orientation scores},
  journal   = {IEEE transactions on medical imaging},
  year      = {2016},
  volume    = {35},
  number    = {12},
  pages     = {2631--2644},
  publisher = {IEEE},
}

@Article{Zana2001,
  author  = {F. Zana and J. C. Klein},
  title   = {Segmentation of vessel-like patterns using mathematical morphology and curvature evaluation},
  journal = {IEEE Transactions on Image Processing},
  year    = {2001},
  volume  = {10},
  number  = {7},
  pages   = {1010-1019},
}

@Article{Pinheiro2013,
  author        = {P. H. O. Pinheiro and R. Collobert},
  title         = {Recurrent Convolutional Neural Networks for Scene Parsing},
  journal       = {CoRR},
  year          = {2013},
  volume        = {abs/1306.2795},
  archiveprefix = {arXiv},
  bibsource     = {dblp computer science bibliography, https://dblp.org},
  biburl        = {https://dblp.org/rec/bib/journals/corr/PinheiroC13},
  eprint        = {1306.2795},
  timestamp     = {Mon, 13 Aug 2018 16:47:48 +0200},
}

@InProceedings{Ioffe2015,
  author    = {Ioffe, Sergey and Szegedy, Christian},
  title     = {Batch Normalization: Accelerating Deep Network Training by Reducing Internal Covariate Shift},
  booktitle = {Proceedings of the 32Nd International Conference on International Conference on Machine Learning - Volume 37},
  year      = {2015},
  series    = {ICML'15},
  pages     = {448--456},
}

@InProceedings{Crowther2006,
  author    = {Crowther, Patricia S. and Cox, Robert J.},
  booktitle = {Knowledge-Based Intelligent Information and Engineering Systems},
  title     = {Accuracy of Neural Network Classifiers as a Property of the Size of the Data Set},
  year      = {2006},
  address   = {Berlin, Heidelberg},
  editor    = {Gabrys, Bogdan and Howlett, Robert J. and Jain, Lakhmi C.},
  pages     = {1143--1149},
  publisher = {Springer Berlin Heidelberg},
  abstract  = {It is well-known that the accuracy of a neural network classifier increases as the number of data points in the training set increases. A previous researcher has proposed a general mathematical model that explains the relationship between training sample size and predictive power. We examine this model using artificially generated data sets containing varying numbers of data points and some real world data sets. We find the model works well when large numbers of data points are available for training, but presents practical difficulties when the amount of available data is small and the data set is difficult to classify.},
  isbn      = {978-3-540-46544-7},
}


@article{li2015cross,
  title={A cross-modality learning approach for vessel segmentation in retinal images},
  author={Li, Qiaoliang and Feng, Bowei and Xie, LinPei and Liang, Ping and Zhang, Huisheng and Wang, Tianfu},
  journal={IEEE transactions on medical imaging},
  volume={35},
  number={1},
  pages={109--118},
  year={2015},
  publisher={IEEE}
}

@ARTICLE{Khan2017Anisotropic,
author={T. M. {Khan} and D. G. {Bailey} and M. A. U. {Khan} and Y. {Kong}},
journal={IEEE Transactions on Image Processing},
title={Efficient Hardware Implementation For Fingerprint Image Enhancement Using Anisotropic Gaussian Filter},
year={2017},
volume={26},
number={5},
pages={2116-2126},
keywords={field programmable gate arrays;fingerprint identification;Gaussian processes;image enhancement;image filtering;parallel architectures;real-time systems;resource allocation;hardware implementation;fingerprint image enhancement;real-time image filtering;fingerprint filtering;modified anisotropic Gaussian filter;orthogonal Gaussians;oriented line Gaussian;performance improvement;local image normalization;middle-range reconfigurable FPGA;parallel compute-intensive demands;real-time demands;image-processing time;resource utilization;hardware architecture;Field programmable gate arrays;Hardware;Real-time systems;Estimation;Image enhancement;Fingerprint recognition;Computer architecture;Fingerprint image enhancement;FPGA;oriented gaussian filter},
doi={10.1109/TIP.2017.2671781},
ISSN={1941-0042},
month={May},}
@article{barkana2017performance,
  title={Performance analysis of descriptive statistical features in retinal vessel segmentation via fuzzy logic, ANN, SVM, and classifier fusion},
  author={Barkana, Buket D and Saricicek, Inci and Yildirim, Burak},
  journal={Knowledge-Based Systems},
  volume={118},
  pages={165--176},
  year={2017},
  publisher={Elsevier}
}
@inproceedings{dasgupta2017fully,
  title={A fully convolutional neural network based structured prediction approach towards the retinal vessel segmentation},
  author={Dasgupta, Avijit and Singh, Sonam},
  booktitle={2017 IEEE 14th International Symposium on Biomedical Imaging (ISBI 2017)},
  pages={248--251},
  year={2017},
  organization={IEEE}
}
@article{liskowski2016segmenting,
  title={Segmenting retinal blood vessels with deep neural networks},
  author={Liskowski, Pawe{\l} and Krawiec, Krzysztof},
  journal={IEEE transactions on medical imaging},
  volume={35},
  number={11},
  pages={2369--2380},
  year={2016},
  publisher={IEEE}
}
@article{aslani2016new,
  title={A new supervised retinal vessel segmentation method based on robust hybrid features},
  author={Aslani, Shahab and Sarnel, Haldun},
  journal={Biomedical Signal Processing and Control},
  volume={30},
  pages={1--12},
  year={2016},
  publisher={Elsevier}
}

@article{matthews1975,
	title = {Comparison of the predicted and observed secondary structure of T4 phage lysozyme},
	journal = {Biochimica et Biophysica Acta (BBA) - Protein Structure},
	volume = {405},
	number = {2},
	pages = {442-451},
	year = {1975},
	issn = {0005-2795},
	author = {B.W. Matthews}
}

@article{orlando2016discriminatively,
  title={A discriminatively trained fully connected conditional random field model for blood vessel segmentation in fundus images},
  author={Orlando, Jos{\'e} Ignacio and Prokofyeva, Elena and Blaschko, Matthew B},
  journal={IEEE Transactions on Biomedical Engineering},
  volume={64},
  number={1},
  pages={16--27},
  year={2016},
  publisher={IEEE}
}
@article{son2017retinal,
  title={Retinal vessel segmentation in fundoscopic imaages with generative adversarial networks},
  author={Son, Jaemin and Park, Sang Jun and Jung, Kyu-Hwan},
  journal={arXiv preprint arXiv:1706.09318},
  year={2017}
}
@article{alom2018recurrent,
  title={Recurrent residual convolutional neural network based on u-net (r2u-net) for medical image segmentation},
  author={Alom, Md Zahangir and Hasan, Mahmudul and Yakopcic, Chris and Taha, Tarek M and Asari, Vijayan K},
  journal={arXiv preprint arXiv:1802.06955},
  year={2018}
}
@article{hu2018retinal,
  title={Retinal vessel segmentation of color fundus images using multiscale convolutional neural network with an improved cross-entropy loss function},
  author={Hu, Kai and Zhang, Zhenzhen and Niu, Xiaorui and Zhang, Yuan and Cao, Chunhong and Xiao, Fen and Gao, Xieping},
  journal={Neurocomputing},
  volume={309},
  pages={179--191},
  year={2018},
  publisher={Elsevier}
}
@article{oliveira2018retinal,
  title={Retinal vessel segmentation based on fully convolutional neural networks},
  author={Oliveira, Am{\'e}rico and Pereira, S{\'e}rgio and Silva, Carlos A},
  journal={Expert Systems with Applications},
  volume={112},
  pages={229--242},
  year={2018},
  publisher={Elsevier}
}
@inproceedings{guo2018automatic,
  title={Automatic Retinal Blood Vessel Segmentation Based on Multi-Level Convolutional Neural Network},
  author={Guo, Jinnan and Ren, Shiwei and Shi, Yueting and Wang, Haoyu},
  booktitle={2018 11th International Congress on Image and Signal Processing, BioMedical Engineering and Informatics (CISP-BMEI)},
  pages={1--5},
  year={2018},
  organization={IEEE}
}
@article{jiang2018retinal,
  title={Retinal blood vessel segmentation using fully convolutional network with transfer learning},
  author={Jiang, Zhexin and Zhang, Hao and Wang, Yi and Ko, Seok-Bum},
  journal={Computerized Medical Imaging and Graphics},
  volume={68},
  pages={1--15},
  year={2018},
  publisher={Elsevier}
}
@article{guo2018retinal,
  title={A retinal vessel detection approach using convolution neural network with reinforcement sample learning strategy},
  author={Guo, Yanhui and Budak, {\"U}mit and Vespa, Lucas J and Khorasani, Elham and {\c{S}}eng{\"u}r, Abdulkadir},
  journal={Measurement},
  volume={125},
  pages={586--591},
  year={2018},
  publisher={Elsevier}
}
@article{arguello2018gpu,
  title={GPU-based segmentation of retinal blood vessels},
  author={Arg{\"u}ello, Francisco and Vilari{\~n}o, David L and Heras, Dora B and Nieto, Alejandro},
  journal={Journal of Real-Time Image Processing},
  volume={14},
  number={4},
  pages={773--782},
  year={2018},
  publisher={Springer}
}
@article{li2019connection,
  title={Connection Sensitive Attention U-NET for Accurate Retinal Vessel Segmentation},
  author={Li, Ruirui and Li, Mingming and Li, Jiacheng},
  journal={arXiv preprint arXiv:1903.05558},
  year={2019}
 }

@article{yan2017skeletal,
  title={A skeletal similarity metric for quality evaluation of retinal vessel segmentation},
  author={Yan, Zengqiang and Yang, Xin and Cheng, Kwang-Ting},
  journal={IEEE transactions on medical imaging},
  volume={37},
  number={4},
  pages={1045--1057},
  year={2017},
  publisher={IEEE}
}
@article{jiang2019retinal,
  title={Retinal Vessels Segmentation Based on Dilated Multi-Scale Convolutional Neural Network},
  author={Jiang, Yun and Tan, Ning and Peng, Tingting and Zhang, Hai},
  journal={arXiv preprint arXiv:1904.05644},
  year={2019}
}
@article{singh2016retinal,
  title={Retinal blood vessels segmentation by using Gumbel probability distribution function based matched filter},
  author={Singh, Nagendra Pratap and Srivastava, Rajeev},
  journal={Computer methods and programs in biomedicine},
  volume={129},
  pages={40--50},
  year={2016},
  publisher={Elsevier}
}
@inproceedings{kumar2016retinal,
  title={Retinal blood vessel segmentation using matched filter and laplacian of gaussian},
  author={Kumar, Debamita and Pramanik, Ankita and Kar, Sudeshna Sil and Maity, Santi P},
  booktitle={2016 International Conference on Signal Processing and Communications (SPCOM)},
  pages={1--5},
  year={2016},
  organization={IEEE}
}
@inproceedings{rodrigues2016retinal,
  title={Retinal vessel segmentation using parallel grayscale skeletonization algorithm and mathematical morphology},
  author={Rodrigues, Jardel and Bezerra, Nivando},
  booktitle={2016 29th SIBGRAPI Conference on Graphics, Patterns and Images (SIBGRAPI)},
  pages={17--24},
  year={2016},
  organization={IEEE}
}
@article{zhang2016robust,
  title={Robust retinal vessel segmentation via locally adaptive derivative frames in orientation scores},
  author={Zhang, Jiong and Dashtbozorg, Behdad and Bekkers, Erik and Pluim, Josien PW and Duits, Remco and ter Haar Romeny, Bart M},
  journal={IEEE transactions on medical imaging},
  volume={35},
  number={12},
  pages={2631--2644},
  year={2016},
  publisher={IEEE}
}
@article{oliveira2016unsupervised,
  title={Unsupervised retinal vessel segmentation using combined filters},
  author={Oliveira, Wendeson S and Teixeira, Joyce Vitor and Ren, Tsang Ing and Cavalcanti, George DC and Sijbers, Jan},
  journal={PloS one},
  volume={11},
  number={2},
  pages={e0149943},
  year={2016},
  publisher={Public Library of Science}
}
@article{bahadarkhan2016morphological,
  title={A morphological hessian based approach for retinal blood vessels segmentation and denoising using region based otsu thresholding},
  author={BahadarKhan, Khan and Khaliq, Amir A and Shahid, Muhammad},
  journal={PloS one},
  volume={11},
  number={7},
  pages={e0158996},
  year={2016},
  publisher={Public Library of Science}
}
@article{rodrigues2017segmentation,
  title={Segmentation of optic disc and blood vessels in retinal images using wavelets, mathematical morphology and Hessian-based multi-scale filtering},
  author={Rodrigues, Luiz Carlos and Marengoni, Maur{\'\i}cio},
  journal={Biomedical Signal Processing and Control},
  volume={36},
  pages={39--49},
  year={2017},
  publisher={Elsevier}
}
@article{neto2017unsupervised,
  title={An unsupervised coarse-to-fine algorithm for blood vessel segmentation in fundus images},
  author={Neto, Luiz C{\^a}mara and Ramalho, Geraldo LB and Neto, Jeov{\'a} FS Rocha and Veras, Rodrigo MS and Medeiros, F{\'a}tima NS},
  journal={Expert Systems with Applications},
  volume={78},
  pages={182--192},
  year={2017},
  publisher={Elsevier}
}
@article{karn2018robust,
  title={Robust retinal blood vessel segmentation using hybrid active contour model},
  author={Karn, Prakash Kumar and Biswal, Birendra and Samantaray, Subhransu Ranjan},
  journal={IET Image Processing},
  volume={13},
  number={3},
  pages={440--450},
  year={2018},
  publisher={IET}
}
@article{aguirre2018blood,
  title={Blood vessel segmentation in retinal fundus images using Gabor filters, fractional derivatives, and Expectation Maximization},
  author={Aguirre-Ramos, Hugo and Avina-Cervantes, Juan Gabriel and Cruz-Aceves, Ivan and Ruiz-Pinales, Jos{\'e} and Ledesma, Sergio},
  journal={Applied Mathematics and Computation},
  volume={339},
  pages={568--587},
  year={2018},
  publisher={Elsevier}
}
@article{khan2018robust,
  title={A robust technique based on {VLM} and {Frangi} filter for retinal vessel extraction and denoising},
  author={Khan, Khan Bahadar and Khaliq, Amir A and Jalil, Abdul and Shahid, Muhammad},
  journal={PLoS One},
  volume={13},
  number={2},
  pages={e0192203},
  year={2018},
  publisher={Public Library of Science}
}
@article{hashemzadeh2019retinal,
  title={Retinal Blood Vessel Extraction Employing Effective Image Features and Combination of Supervised and Unsupervised Machine Learning Methods},
  author={Hashemzadeh, Mahdi and Azar, Baharak Adlpour},
  journal={Artificial intelligence in medicine},
  year={2019},
  publisher={Elsevier}
}
@article{bressler1988age,
  title={Age-related macular degeneration},
  author={Bressler, Neil M and Bressler, Susan B and Fine, Stuart L},
  journal={Survey of ophthalmology},
  volume={32},
  number={6},
  pages={375--413},
  year={1988},
  publisher={Elsevier}
}
@article{tang2011inflammation,
  title={Inflammation in diabetic retinopathy},
  author={Tang, Johnny and Kern, Timothy S},
  journal={Progress in retinal and eye research},
  volume={30},
  number={5},
  pages={343--358},
  year={2011},
  publisher={Elsevier}
}
@article{davidson2007diabetic,
  title={How the diabetic eye loses vision},
  author={Davidson, Jaime A and Ciulla, Thomas A and McGill, Janet B and Kles, Keri A and Anderson, Pamela W},
  journal={Endocrine},
  volume={32},
  number={1},
  pages={107--116},
  year={2007},
  publisher={Springer}
}
%============ newly added paperssss=============

@Article{Lam2010,
  author      = {B. S. Y. Lam and Y. Gao and A. W. Liew},
  title       = {General Retinal Vessel Segmentation Using Regularization-Based Multiconcavity Modeling},
  journal     = {IEEE Transactions on Medical Imaging},
  year        = {2010},
  volume      = {29},
  number      = {7},
  pages       = {1369--1381},
  issn        = {0278-0062},
  call-number = {29},
  keywords    = {biomedical optical imaging, blood vessels, eye, image denoising, image segmentation, medical image processing, retinal vessel segmentation, regularization based multiconcavity modeling, blood vessel detection, retinal images, bright lesions, dark lesions, differentiable concavity measure, perceptive space, line shape concavity measure, lesion intensity structure, line shaped vessels, unevenly distributed noise, retinal image spherical intensity variation, Retinal vessels, Retina, Lesions, Image segmentation, Blood vessels, Biomedical imaging, Extraterrestrial measurements, Noise measurement, Statistical distributions, Humans, Multiconcavity modeling, perceptive transform, regularization, retina image, retinal vessel segmentation, Algorithms, Computer Simulation, Humans, Image Enhancement, Image Interpretation, Computer-Assisted, Information Storage and Retrieval, Models, Biological, Pattern Recognition, Automated, Reproducibility of Results, Retinal Vessels, Retinoscopy, Sensitivity and Specificity},
}
@Article{Miri2011,
  author      = {Miri, M. S. and Mahloojifar, A.},
  title       = {Retinal Image Analysis Using Curvelet Transform and Multistructure Elements Morphology by Reconstruction},
  journal     = {IEEE Transactions on Biomedical Engineering},
  year        = {2011},
  volume      = {58},
  number      = {5},
  pages       = {1183--1192},
  issn        = {0018-9294},
  call-number = {58},
  keywords    = {biomedical optical imaging, blood vessels, curvelet transforms, eye, image reconstruction, image segmentation, medical image processing, patient diagnosis, retinal image analysis, curvelet transform, image reconstruction, ocular fundus operations, human recognition, early stage disease detection, diabetes, retinal blood vessels, image segmentation, multistructure elements method, morphology operators, connected components analysis, DRIVE, blood vessel detection, Image edge detection, Retina, Transforms, Image reconstruction, Morphology, Blood vessels, Biomedical imaging, Blood vessel segmentation, curvelet transform, morphology operators by reconstruction, multistructure elements morphology, retinal image, Algorithms, Databases, Factual, Diagnostic Techniques, Ophthalmological, Fundus Oculi, Humans, Image Processing, Computer-Assisted, Models, Statistical, Retinal Vessels},
}

@Article{You2011,
  author   = {X. You and Q. Peng and Y. Yuan and Y. Cheung and J. Lei},
  title    = {Segmentation of retinal blood vessels using the radial projection and semi-supervised approach},
  journal  = {Pattern Recognition},
  year     = {2011},
  volume   = {44},
  number   = {10},
  pages    = {2314 - 2324},
  issn     = {0031-3203},
  note     = {Semi-Supervised Learning for Visual Content Analysis and Understanding},
  doi      = {https://doi.org/10.1016/j.patcog.2011.01.007},
  keywords = {Radial projection, Retinal images, Steerable complex wavelet},
  url      = {http://www.sciencedirect.com/science/article/pii/S0031320311000161},
}


@ARTICLE{Marin2011,
author={D. Marin and A. Aquino and M. E. Gegundez-Arias and J. M. Bravo},
journal={IEEE Transactions on Medical Imaging},
title={A New Supervised Method for Blood Vessel Segmentation in Retinal Images by Using Gray-Level and Moment Invariants-Based Features},
year={2011},
volume={30},
number={1},
pages={146-158}
}
@Article{Zhang2010,
  author   = {Zhang, B. and Zhang, L. and Zhang, L. and Karray, F.},
  title    = {Retinal vessel extraction by matched filter with first-order derivative of Gaussian},
  journal  = {Computers in Biology and Medicine},
  year     = {2010},
  volume   = {40},
  number   = {4},
  pages    = {438--445},
  month    = apr,
  issn     = {0010-4825},
  keywords = {Retinal image segmentation, Vessel detection, Matched filter, Line detection},
  url      = {http://www.sciencedirect.com/science/article/pii/S0010482510000302},
}

@ARTICLE{Soares2006,
author={J. V. B. Soares and J. J. G. Leandro and R. M. Cesar and H. F. Jelinek and M. J. Cree},
journal={IEEE Transactions on Medical Imaging},
title={Retinal vessel segmentation using the 2-D Gabor wavelet and supervised classification},
year={2006},
volume={25},
number={9},
pages={1214-1222}
}
@ARTICLE{Ricci2007,
author={E. Ricci and R. Perfetti},
journal={IEEE Transactions on Medical Imaging},
title={Retinal Blood Vessel Segmentation Using Line Operators and Support Vector Classification},
year={2007},
volume={26},
number={10},
pages={1357-1365}
}


@inproceedings{niemeijer2004,
  title={Comparative study of retinal vessel segmentation methods on a new publicly available database},
  author={Niemeijer, Meindert and Staal, Joes and van Ginneken, Bram and Loog, Marco and Abramoff, Michael D},
  booktitle={Medical imaging 2004: image processing},
  volume={5370},
  pages={648--657},
  year={2004},
  organization={International Society for Optics and Photonics}
}

@InProceedings{Wang2019,
  author    = {Wang, B. and Qiu, S. and He H.},
  booktitle = {Medical Image Computing and Computer Assisted Intervention – MICCAI 2019},
  title     = {Dual Encoding U-Net for Retinal Vessel Segmentation},
  year      = {2019},
}


@article{dai2016retinal,
  title={Retinal fundus image enhancement using the normalized convolution and noise removing},
  author={Dai, Peishan and Sheng, Hanwei and Zhang, Jianmei and Li, Ling and Wu, Jing and Fan, Min},
  journal={International journal of biomedical imaging},
  volume={2016},
  year={2016},
  publisher={Hindawi}
}

@article{hosseinkhani2017real,
  title={Real-time impulse noise removal from MR images for radiosurgery applications},
  author={HosseinKhani, Zohreh and Hajabdollahi, Mohsen and Karimi, Nader and Soroushmehr, SM and Shirani, Shahram and Samavi, Shadrokh and Najarian, Kayvan},
  journal={arXiv preprint arXiv:1707.05975},
  year={2017}
}

@inproceedings{sharp2008application,
  title={Application of sparse signal recovery to pilot-assisted channel estimation},
  author={Sharp, Matthew and Scaglione, Anna},
  booktitle={2008 IEEE International Conference on Acoustics, Speech and Signal Processing},
  pages={3469--3472},
  year={2008},
  organization={IEEE}
}

@article{parvaresh2008recovering,
  title={Recovering sparse signals using sparse measurement matrices in compressed DNA microarrays},
  author={Parvaresh, Farzad and Vikalo, Haris and Misra, Sidhant and Hassibi, Babak},
  journal={IEEE Journal of Selected Topics in Signal Processing},
  volume={2},
  number={3},
  pages={275--285},
  year={2008},
  publisher={IEEE}
}

@article{dabov2007BM3D,
  title={Image denoising by sparse 3-D transform-domain collaborative filtering},
  author={Dabov, Kostadin and Foi, Alessandro and Katkovnik, Vladimir and Egiazarian, Karen},
  journal={IEEE Transactions on image processing},
  volume={16},
  number={8},
  pages={2080--2095},
  year={2007},
  publisher={IEEE}
}

@article{aghagolzadeh1992transform,
  title={Transform image enhancement},
  author={Aghagolzadeh, Sabzali and Ersoy, Okan K},
  journal={Optical Engineering},
  volume={31},
  number={3},
  pages={614--627},
  year={1992},
  publisher={International Society for Optics and Photonics}
}

@inproceedings{dabov2007joint,
  title={Joint image sharpening and denoising by 3D transform-domain collaborative filtering},
  author={Dabov, Kostadin and Foi, Alessandro and Katkovnik, Vladimir and Egiazarian, Karen},
  booktitle={Proc. 2007 Int. TICSP Workshop Spectral Meth. Multirate Signal Process., SMMSP},
  volume={2007},
  year={2007},
  organization={Citeseer}
}
@Conference{Hunter2005,
  author    = {Hunter, Andrew and Lowell, James and Ryder, Robert and Basu, Ansu and Steel, David},
  title     = {Tram-Line filtering for retinal vessel segmentation},
  booktitle = {3rd European Medical and Biological Engineering Conference},
  year      = {2005},
  pages     = {20-24},
}

@InProceedings{Frangi1998,
  author    = {Frangi, Alejandro F. and Niessen, Wiro J. and Vincken, Koen L. and Viergever, Max A.},
  title     = {Multiscale vessel enhancement filtering},
  booktitle = {Medical Image Computing and Computer-Assisted Intervention --- MICCAI'98},
  year      = {1998},
  editor    = {Wells, William M. and Colchester, Alan and Delp, Scott},
  pages     = {130--137},
  address   = {Berlin, Heidelberg},
  publisher = {Springer Berlin Heidelberg},
  abstract  = {The multiscale second order local structure of an image (Hessian) is examined with the purpose of developing a vessel enhancement filter. A vesselness measure is obtained on the basis of all eigenvalues of the Hessian. This measure is tested on two dimensional DSA and three dimensional aortoiliac and cerebral MRA data. Its clinical utility is shown by the simultaneous noise and background suppression and vessel enhancement in maximum intensity projections and volumetric displays.},
  isbn      = {978-3-540-49563-5},
}

@Article{Xiao2011,
  author   = {Changyan Xiao and Marius Staring and Denis Shamonin and Johan H.C. Reiber and Jan Stolk and Berend C. Stoel},
  title    = {A strain energy filter for 3D vessel enhancement with application to pulmonary CT images},
  journal  = {Medical Image Analysis},
  year     = {2011},
  volume   = {15},
  number   = {1},
  pages    = {112 - 124},
  issn     = {1361-8415},
  abstract = {The traditional Hessian-related vessel filters often suffer from detecting complex structures like bifurcations due to an over-simplified cylindrical model. To solve this problem, we present a shape-tuned strain energy density function to measure vessel likelihood in 3D medical images. This method is initially inspired by established stress–strain principles in mechanics. By considering the Hessian matrix as a stress tensor, the three invariants from orthogonal tensor decomposition are used independently or combined to formulate distinctive functions for vascular shape discrimination, brightness contrast and structure strength measuring. Moreover, a mathematical description of Hessian eigenvalues for general vessel shapes is obtained, based on an intensity continuity assumption, and a relative Hessian strength term is presented to ensure the dominance of second-order derivatives as well as suppress undesired step-edges. Finally, we adopt the multi-scale scheme to find an optimal solution through scale space. The proposed method is validated in experiments with a digital phantom and non-contrast-enhanced pulmonary CT data. It is shown that our model performed more effectively in enhancing vessel bifurcations and preserving details, compared to three existing filters.},
  doi      = {https://doi.org/10.1016/j.media.2010.08.003},
  keywords = {Vessel enhancement, Strain energy density, Shape discrimination, Pulmonary image analysis},
}

@Article{nguyen2013effective,
  author    = {Nguyen, Uyen TV and Bhuiyan, Alauddin and Park, Laurence AF and Ramamohanarao, Kotagiri},
  title     = {An effective retinal blood vessel segmentation method using multi-scale line detection},
  journal   = {Pattern recognition},
  year      = {2013},
  volume    = {46},
  number    = {3},
  pages     = {703--715},
  publisher = {Elsevier},
}

@Article{ridler1978picture,
  author  = {Ridler, TW and Calvard, S and others},
  journal = {IEEE transactions on Systems, Man and Cybernetics},
  title   = {Picture thresholding using an iterative selection method},
  year    = {1978},
  number  = {8},
  pages   = {630--632},
  volume  = {8},
  file    = {:ridler1978picture - Picture Thresholding Using an Iterative Selection Method.bib:bib;:citation-335600875.bib:bib},
}

@Article{Wang2019circumscribed,
author="Wang, Weihua
and Wang, Weiqing
and Hu, Zhangping",
title="Segmenting retinal vessels with revised top-bottom-hat transformation and flattening of minimum circumscribed ellipse",
journal="Medical {\&} Biological Engineering {\&} Computing",
year="2019",
month="Jul",
volume="57",
number="7",
pages="1481--1496"}

@article{ZHOU2020Markov,
title = "A new robust method for blood vessel segmentation in retinal fundus images based on weighted line detector and hidden Markov model",
journal = "Computer Methods and Programs in Biomedicine",
volume = "187",
pages = "105231",
year = "2020",
issn = "0169-2607",
author = "Chao Zhou and Xiaogang Zhang and Hua Chen"}

@article{SHIN2019Graphical,
title = "Deep vessel segmentation by learning graphical connectivity",
journal = "Medical Image Analysis",
volume = "58",
pages = "101556",
year = "2019",
author = "Seung Yeon Shin and Soochahn Lee and Il Dong Yun and Kyoung Mu Lee"}

@ARTICLE{Zhao2019Synthesis,
author={H. {Zhao} and H. {Li} and S. {Maurer-Stroh} and Y. {Guo} and Q. {Deng} and L. {Cheng}},
journal={IEEE Transactions on Medical Imaging},
title={Supervised Segmentation of Un-Annotated Retinal Fundus Images by Synthesis},
year={2019},
volume={38},
number={1},
pages={46-56}}

@article{Owen2009,
    author = {Owen, Christopher G. and Rudnicka, Alicja R. and Mullen, Robert and Barman, Sarah A. and Monekosso, Dorothy and Whincup, Peter H. and Ng, Jeffrey and Paterson, Carl},
    title = {Measuring Retinal Vessel Tortuosity in 10-Year-Old Children: Validation of the Computer-Assisted Image Analysis of the Retina (CAIAR) Program},
    journal = {Investigative Ophthalmology \& Visual Science},
    volume = {50},
    number = {5},
    pages = {2004-2010},
    year = {2009}
}

@Article{knutsson1983anisotropic,
  author    = {Knutsson, Hans and Wilson, Roland and Granlund, G{\"o}sta},
  title     = {Anisotropic nonstationary image estimation and its applications: Part I-Restoration of noisy images},
  journal   = {IEEE Transactions on Communications},
  year      = {1983},
  volume    = {31},
  number    = {3},
  pages     = {388--397},
  publisher = {IEEE},
}

@Article{Jeswal2019,
  author   = {Jeswal, S. K. and Chakraverty, S.},
  journal  = {Archives of Computational Methods in Engineering},
  title    = {Recent Developments and Applications in Quantum Neural Network: A Review},
  year     = {2019},
  issn     = {1886-1784},
  month    = sep,
  number   = {4},
  pages    = {793--807},
  volume   = {26},
  abstract = {Quantum neural network is a useful tool which has seen more development over the years mainly after twentieth century. Like artificial neural network (ANN), a novel, useful and applicable concept has been proposed recently which is known as quantum neural network (QNN). QNN has been developed combining the basics of ANN with quantum computation paradigm which is superior than the traditional ANN. QNN is being used in computer games, function approximation, handling big data etc. Algorithms of QNN are also used in modelling social networks, associative memory devices, and automated control systems etc. Different models of QNN has been proposed by different researchers throughout the world but systematic study of these models have not been done till date. Moreover, application of QNN may also be seen in some of the related research papers. As such, this paper includes different models which have been developed and further the implement of the same in various applications. In order to understand the powerfulness of QNN, few results and reasons are incorporated to show that these new models are more useful and efficient than traditional ANN.},
  groups   = {[tariq:]},
  refid    = {Jeswal2019},
  url      = {https://doi.org/10.1007/s11831-018-9269-0},
}

@Article{Chen2017,
  author   = {Chen, Jialin and Wang, Lingli and Charbon, Edoardo},
  journal  = {Quantum Information Processing},
  title    = {A quantum-implementable neural network model},
  year     = {2017},
  issn     = {1573-1332},
  month    = aug,
  number   = {10},
  pages    = {245},
  volume   = {16},
  abstract = {A quantum-implementable neural network, namely quantum probability neural network (QPNN) model, is proposed in this paper. QPNN can use quantum parallelism to trace all possible network states to improve the result. Due to its unique quantum nature, this model is robust to several quantum noises under certain conditions, which can be efficiently implemented by the qubus quantum computer. Another advantage is that QPNN can be used as memory to retrieve the most relevant data and even to generate new data. The MATLAB experimental results of Iris data classification and MNIST handwriting recognition show that much less neuron resources are required in QPNN to obtain a good result than the classical feedforward neural network. The proposed QPNN model indicates that quantum effects are useful for real-life classification tasks.},
  groups   = {tariq:6},
  refid    = {Chen2017},
  url      = {https://doi.org/10.1007/s11128-017-1692-x},
}

@Misc{,
  title = {S0950705119301984.ris},
  file  = {:C\:/Users/61420/Downloads/S0950705119301984.ris:ris},
}

@Article{Guo2019,
  author   = {Song Guo and Kai Wang and Hong Kang and Yujun Zhang and Yingqi Gao and Tao Li},
  journal  = {International Journal of Medical Informatics},
  title    = {{BTS-DSN}: Deeply supervised neural network with short connections for retinal vessel segmentation},
  year     = {2019},
  issn     = {1386-5056},
  pages    = {105-113},
  volume   = {126},
  abstract = {Background and objective
The condition of vessel of the human eye is an important factor for the diagnosis of ophthalmological diseases. Vessel segmentation in fundus images is a challenging task due to complex vessel structure, the presence of similar structures such as microaneurysms and hemorrhages, micro-vessel with only one to several pixels wide, and requirements for finer results.
Methods
In this paper, we present a multi-scale deeply supervised network with short connections (BTS-DSN) for vessel segmentation. We used short connections to transfer semantic information between side-output layers. Bottom-top short connections pass low level semantic information to high level for refining results in high-level side-outputs, and top-bottom short connection passes much structural information to low level for reducing noises in low-level side-outputs. In addition, we employ cross-training to show that our model is suitable for real world fundus images.
Results
The proposed BTS-DSN has been verified on DRIVE, STARE and CHASE_DB1 datasets, and showed competitive performance over other state-of-the-art methods. Specially, with patch level input, the network achieved 0.7891/0.8212 sensitivity, 0.9804/0.9843 specificity, 0.9806/0.9859 AUC, and 0.8249/0.8421 F1-score on DRIVE and STARE, respectively. Moreover, our model behaves better than other methods in cross-training experiments.
Conclusions
BTS-DSN achieves competitive performance in vessel segmentation task on three public datasets. It is suitable for vessel segmentation. The source code of our method is available at: https://github.com/guomugong/BTS-DSN.},
  file     = {:Guo2019 - BTS DSN_ Deeply Supervised Neural Network with Short Connections for Retinal Vessel Segmentation.bib:bib},
  keywords = {Vessel segmentation, Fundus image, Deep supervision, Short connection},
}

@InProceedings{Ma2019,
  author    = {Ma, Wenao and Yu, Shuang and Ma, Kai and Wang, Jiexiang and Ding, Xinghao and Zheng, Yefeng},
  booktitle = {Medical Image Computing and Computer Assisted Intervention – MICCAI 2019},
  title     = {Multi-Task Neural Networks with Spatial Activation for Retinal Vessel Segmentation and Artery/Vein Classification},
  year      = {2019},
  month     = {09},
}

@Article{,
  author = {Wang, B. and Qiu, S. and He H.},
}

@InBook{Wu2019,
  author  = {Wu, Yicheng and Xia, Yong and Song, Yang and Zhang, Donghao and Liu, Dongnan and Zhang, Chaoyi and Cai, Weidong},
  chapter = {Medical Image Computing and Computer Assisted Intervention – MICCAI 2019},
  pages   = {264-272},
  title   = {Vessel-Net: Retinal Vessel Segmentation Under Multi-path Supervision},
  year    = {2019},
  isbn    = {978-3-030-32238-0},
  month   = {10},
  doi     = {10.1007/978-3-030-32239-7_30},
  file    = {:Wu2019 - Vessel Net_ Retinal Vessel Segmentation under Multi Path Supervision.bib:bib},
}

@Article{Wang2020,
  author  = {Dongyi Wang and Ayman Haytham and Jessica Pottenburgh and Osamah Saeedi and Yang Tao},
  journal = {IEEE Journal ofBiomedical and Health Informatics},
  title   = {Hard Attention Net for Automatic Retinal VesselSegmentation},
  year    = {2020},
  doi     = {10.1109/JBHI.2020.3002985},
}

@Article{Yin2020,
  author   = {P. {Yin} and R. {Yuan} and Y. {Cheng} and Q. {Wu}},
  journal  = {IEEE Access},
  title    = {Deep Guidance Network for Biomedical Image Segmentation},
  year     = {2020},
  issn     = {2169-3536},
  pages    = {116106-116116},
  volume   = {8},
  abstract = {Segmentation of 2D images is a fundamental problem for biomedical image analysis. The most widely used architecture for biomedical image segmentation is U-Net. U-Net introduces skip-connections to restore the spatial information loss caused by down-sampling operations. However, for some tasks such as the retinal vessel segmentation, the loss information of structure can not be fully recovered since the vessels is merely a curve line that can not be detected after several convolutions. In this paper, we introduce a deep guidance network to segment the biomedical image. Our proposed network consists of a guided image filter module to restore the structure information through the guidance image. Our method enables end to end training and fast inference (43ms for one image). We conduct extensive experiments for the task of vessel segmentation and optic disc and cup segmentation. The experiments on four publicly available datasets: ORIGA, REFUGE, DRIVE, and CHASEDB1 verify the effectiveness of our method.},
  doi      = {10.1109/ACCESS.2020.3002835},
  keywords = {Image segmentation;Biomedical optical imaging;Optical imaging;Optical filters;Retina;Adaptive optics;Biomedical image segmentation;semantic segmentation;guided filter},
}

@Article{Gu2019,
  author   = {Z. {Gu} and J. {Cheng} and H. {Fu} and K. {Zhou} and H. {Hao} and Y. {Zhao} and T. {Zhang} and S. {Gao} and J. {Liu}},
  journal  = {IEEE Transactions on Medical Imaging},
  title    = {CE-Net: Context Encoder Network for 2D Medical Image Segmentation},
  year     = {2019},
  issn     = {1558-254X},
  month    = {Oct},
  number   = {10},
  pages    = {2281-2292},
  volume   = {38},
  abstract = {Medical image segmentation is an important step in medical image analysis. With the rapid development of a convolutional neural network in image processing, deep learning has been used for medical image segmentation, such as optic disc segmentation, blood vessel detection, lung segmentation, cell segmentation, and so on. Previously, U-net based approaches have been proposed. However, the consecutive pooling and strided convolutional operations led to the loss of some spatial information. In this paper, we propose a context encoder network (CE-Net) to capture more high-level information and preserve spatial information for 2D medical image segmentation. CE-Net mainly contains three major components: a feature encoder module, a context extractor, and a feature decoder module. We use the pretrained ResNet block as the fixed feature extractor. The context extractor module is formed by a newly proposed dense atrous convolution block and a residual multi-kernel pooling block. We applied the proposed CE-Net to different 2D medical image segmentation tasks. Comprehensive results show that the proposed method outperforms the original U-Net method and other state-of-the-art methods for optic disc segmentation, vessel detection, lung segmentation, cell contour segmentation, and retinal optical coherence tomography layer segmentation.},
  doi      = {10.1109/TMI.2019.2903562},
  keywords = {blood vessels;convolutional neural nets;eye;feature extraction;image segmentation;learning (artificial intelligence);lung;medical image processing;CE-Net;context encoder network;2D medical image segmentation;medical image analysis;optic disc segmentation;lung segmentation;U-Net method;convolutional neural network;deep learning;Image segmentation;Feature extraction;Convolution;Biomedical optical imaging;Optical imaging;Computed tomography;Medical image segmentation;deep learning;context encoder network},
}

@Article{Arsalan2019,
  author  = {Muhammad Arsalan and Muhamamd Oqais and tahir Mahmood and Se Woon Cho and Kang Ryoung Park},
  journal = {Journal of Clinical Medicine},
  title   = {Aiding the Diagnosis of Diabetic and Hypertensive Retinopathy Using Artificial Intelligence-Based Semantic Segmentation},
  year    = {2019},
  number  = {9},
  volume  = {8},
  doi     = {10.3390/jcm8091446},
}

@Article{Fraz2012,
  author   = {M. M. {Fraz} and P. {Remagnino} and A. {Hoppe} and B. {Uyyanonvara} and A. R. {Rudnicka} and C. G. {Owen} and S. A. {Barman}},
  journal  = {IEEE Transactions on Biomedical Engineering},
  title    = {An Ensemble Classification-Based Approach Applied to Retinal Blood Vessel Segmentation},
  year     = {2012},
  issn     = {1558-2531},
  number   = {9},
  pages    = {2538-2548},
  volume   = {59},
  abstract = {This paper presents a new supervised method for segmentation of blood vessels in retinal photographs. This method uses an ensemble system of bagged and boosted decision trees and utilizes a feature vector based on the orientation analysis of gradient vector field, morphological transformation, line strength measures, and Gabor filter responses. The feature vector encodes information to handle the healthy as well as the pathological retinal image. The method is evaluated on the publicly available DRIVE and STARE databases, frequently used for this purpose and also on a new public retinal vessel reference dataset CHASE_DB1 which is a subset of retinal images of multiethnic children from the Child Heart and Health Study in England (CHASE) dataset. The performance of the ensemble system is evaluated in detail and the incurred accuracy, speed, robustness, and simplicity make the algorithm a suitable tool for automated retinal image analysis.},
  doi      = {10.1109/TBME.2012.2205687},
  keywords = {Retina;Biomedical imaging;Training;Blood vessels;Databases;Lesions;Vectors;Ensemble classification;medical image analysis;retinal blood vessels;segmentation;Algorithms;Area Under Curve;Child;Databases, Factual;Decision Trees;Humans;Image Processing, Computer-Assisted;Pattern Recognition, Automated;Retinal Vessels},
}
@InProceedings{Zhao2018,
author="Zhao, Yitian
and Xie, Jianyang
and Su, Pan
and Zheng, Yalin
and Liu, Yonghuai
and Cheng, Jun
and Liu, Jiang",
title="Retinal Artery and Vein Classification via Dominant Sets Clustering-Based Vascular Topology Estimation",
booktitle="Medical Image Computing and Computer Assisted Intervention (MICCAI)",
year="2018",
pages="56--64",
abstract="The classification of the retinal vascular tree into arteries and veins is important in understanding the relation between vascular changes and a wide spectrum of diseases. In this paper, we have proposed a novel framework that is capable of making the artery/vein (A/V) distinction in retinal color fundus images. We have successfully adapted the concept of dominant sets clustering and formalize the retinal vessel topology estimation and the A/V classification problem as a pairwise clustering problem. Dominant sets clustering is a graph-theoretic approach that has been proven to work well in data clustering. The proposed approach has been applied to three public databases (INSPIRE, DRIVE and VICAVR) and achieved high accuracies of 91.0{\%}, 91.2{\%}, and 91.0{\%}, respectively. Furthermore, we have made manual annotations of vessel topologies from these databases, and this annotation will be released for public access to facilitate other researchers in the community to do research in the same and related topics.",
isbn="978-3-030-00934-2"
}


@INPROCEEDINGS{Zheng2016,  author={H. {Zheng} and L. {Chang} and T. {Wei} and X. {Qiu} and P. {Lin} and Y. {Wang}},  booktitle={2016 IEEE Conference on Computer Vision and Pattern Recognition Workshops (CVPRW)},   title={Registering Retinal Vessel Images from Local to Global via Multiscale and Multicycle Features},   year={2016},  volume={},  number={},  pages={490-497},}
@ARTICLE{Soomro19,  author={T. A. {Soomro} and A. J. {Afifi} and A. {Ali Shah} and S. {Soomro} and G. A. {Baloch} and L. {Zheng} and M. {Yin} and J. {Gao}},  journal={IEEE Access},   title={Impact of Image Enhancement Technique on {CNN} Model for Retinal Blood Vessels Segmentation},   year={2019},  volume={7},  number={},  pages={158183-158197},}
@ARTICLE{Xiuqin19,  author={P. {Xiuqin} and Q. {Zhang} and H. {Zhang} and S. {Li}},  journal={IEEE Access},   title={A Fundus Retinal Vessels Segmentation Scheme Based on the Improved Deep Learning U-Net Model},   year={2019},  volume={7},  number={},  pages={122634-122643},}

@InProceedings{Ronneberger2015,
author="Ronneberger, Olaf
and Fischer, Philipp
and Brox, Thomas",
title="{U-Net}: Convolutional Networks for Biomedical Image Segmentation",
booktitle="Medical Image Computing and Computer-Assisted Intervention (MICCAI)",
year="2015",
pages="234--241",
abstract="There is large consent that successful training of deep networks requires many thousand annotated training samples. In this paper, we present a network and training strategy that relies on the strong use of data augmentation to use the available annotated samples more efficiently. The architecture consists of a contracting path to capture context and a symmetric expanding path that enables precise localization. We show that such a network can be trained end-to-end from very few images and outperforms the prior best method (a sliding-window convolutional network) on the ISBI challenge for segmentation of neuronal structures in electron microscopic stacks. Using the same network trained on transmitted light microscopy images (phase contrast and DIC) we won the ISBI cell tracking challenge 2015 in these categories by a large margin. Moreover, the network is fast. Segmentation of a 512x512 image takes less than a second on a recent GPU. The full implementation (based on Caffe) and the trained networks are available at http://lmb.informatik.uni-freiburg.de/people/ronneber/u-net.",
isbn="978-3-319-24574-4"
}



@article{Gu2019CENetCE,
  title={{CE-Net}: Context Encoder Network for {2D} Medical Image Segmentation},
  author={Zaiwang Gu and J. Cheng and Huazhu Fu and K. Zhou and Huaying Hao and Yitian Zhao and Tianyang Zhang and Shenghua Gao and Jiang Liu},
  journal={IEEE Transactions on Medical Imaging},
  year={2019},
  volume={38},
  pages={2281-2292}
}

@article{taghanaki2019combo,
  title={Combo loss: Handling input and output imbalance in multi-organ segmentation},
  author={Taghanaki, Saeid Asgari and Zheng, Yefeng and Zhou, S Kevin and Georgescu, Bogdan and Sharma, Puneet and Xu, Daguang and Comaniciu, Dorin and Hamarneh, Ghassan},
  journal={Computerized Medical Imaging and Graphics},
  volume={75},
  pages={24--33},
  year={2019},
  publisher={Elsevier}
}

@Article{,
}

@Article{,
}

@InProceedings{Wang2019a,
  author    = {B. Wang and S. Qiu and H. He},
  booktitle = {Medical Image Computing and Computer Assisted Intervention (MICCAI)},
  title     = {Dual encoding {U-Net} for retinal vesselsegmentation},
  year      = {2019},
  pages     = {84-92},
}

@inproceedings{Szegedy2017,
author = {Szegedy, Christian and Ioffe, Sergey and Vanhoucke, Vincent and Alemi, Alexander A.},
title = {Inception-v4, Inception-ResNet and the Impact of Residual Connections on Learning},
year = {2017},
publisher = {AAAI Press},
booktitle = {Proceedings of the Thirty-First AAAI Conference on Artificial Intelligence},
pages = {4278–4284},
numpages = {7},
location = {San Francisco, California, USA},
series = {AAAI'17}
}

@InProceedings{Zongwei2018,
author="Zhou, Zongwei
and Rahman Siddiquee, Md Mahfuzur
and Tajbakhsh, Nima
and Liang, Jianming",
title="{UNet++}: A Nested {U-Net} Architecture for Medical Image Segmentation",
booktitle="Deep Learning in Medical Image Analysis \& Multimodal Learning for Clinical Decision Support",
year="2018",
pages="3--11"
}

@inproceedings{khan2021residual,
  title={Residual Multiscale Full Convolutional Network (RM-FCN) for High Resolution Semantic Segmentation of Retinal Vasculature},
  author={Khan, Tariq M and Robles-Kelly, Antonio and Naqvi, Syed S and Muhammad, Arsalan},
  booktitle={Structural, Syntactic, and Statistical Pattern Recognition: Joint IAPR International Workshops, S+ SSPR 2020, Padua, Italy, January 21--22, 2021, Proceedings},
  pages={324},
  year={2021},
  organization={Springer Nature}
}

@INPROCEEDINGS{JWang2016,
  author={J. {Wang} and Y. {Yang} and J. {Mao} and Z. {Huang} and C. {Huang} and W. {Xu}},
  booktitle={2016 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  title={CNN-RNN: A Unified Framework for Multi-label Image Classification},
  year={2016},
  volume={},
  number={},
  pages={2285-2294},}

@article{IBTEHAZ202074,
title = "{MultiResUNet}: Rethinking the {U-Net} architecture for multimodal biomedical image segmentation",
journal = "Neural Networks",
volume = "121",
pages = "74-87",
year = "2020",
issn = "0893-6080",
author = "Nabil Ibtehaz and M. Sohel Rahman"}

@inproceedings{azad2019bi,
  title={Bi-directional {ConvLSTM U-net} with Densley connected convolutions},
  author={Azad, Reza and Asadi-Aghbolaghi, Maryam and Fathy, Mahmood and Escalera, Sergio},
  booktitle={IEEE International Conference on Computer Vision Workshops},
  year={2019}
}

@ARTICLE{Yuyi2017MEC,  
author={Mao, Yuyi and You, Changsheng and Zhang, Jun and Huang, Kaibin and Letaief, Khaled B.},  
journal={IEEE Communications Surveys   Tutorials},   
title={A Survey on Mobile Edge Computing: The Communication Perspective},  
year={2017},  
volume={19},  
number={4},  
pages={2322-2358},  
doi={10.1109/COMST.2017.2745201}}

@article{Syed2021URLLC,
author = "Junaid Nawaz Syed and Shree Krishna Sharma and Mohmammad N. Patwary and Md Asaduzzaman",
title = "{Enhanced URLLC-Enabled Edge Computing Framework for Device-Level Innovation in 6G}",
year = "2021",
month = "2",
url = "https://www.techrxiv.org/articles/preprint/Next-Generation_Consumer_Electronics_for_6G_Wireless_Era/13325336",
doi = "10.36227/techrxiv.13325336.v2"
}

@inproceedings{yin2015cloud,
  title={A cloud-based system for automatic glaucoma screening},
  author={Yin, Fengshou and Wong, Damon Wing Kee and Quan, Ying and Yow, Ai Ping and Tan, Ngan Meng and Gopalakrishnan, Kavitha and Lee, Beng Hai and Xu, Yanwu and Zhang, Zhuo and Cheng, Jun and others},
  booktitle={2015 37th Annual International Conference of the IEEE Engineering in Medicine and Biology Society (EMBC)},
  pages={1596--1599},
  year={2015},
  organization={IEEE}
}

@article{Foot2017loss,
author = {Foot, B and Macewen, Caroline},
year = {2017},
month = {01},
pages = {},
title = {Surveillance of sight loss due to delay in ophthalmic treatment or review: Frequency, cause and outcome},
volume = {31},
journal = {Eye},
doi = {10.1038/eye.2017.1}
}

@article{davis2017review,
  title={A review of 145 234 ophthalmic patient episodes lost to follow-up},
  author={Davis, A and Baldwin, A and Hingorani, M and Dwyer, A and Flanagan, D},
  journal={Eye},
  volume={31},
  number={3},
  pages={422--429},
  year={2017},
  publisher={Nature Publishing Group}
}

@INPROCEEDINGS{Ignatov2019mobile,
  author={Ignatov, Andrey and Timofte, Radu and Kulik, Andrei and Yang, Seungsoo and Wang, Ke and Baum, Felix and Wu, Max and Xu, Lirong and Van Gool, Luc},
  booktitle={2019 IEEE/CVF International Conference on Computer Vision Workshop (ICCVW)}, 
  title={AI Benchmark: All About Deep Learning on Smartphones in 2019}, 
  year={2019},
  volume={},
  number={},
  pages={3617-3635},
  doi={10.1109/ICCVW.2019.00447}}
  
@article{crosby2012retinal,
  title={Retinal vascular calibre, geometry and progression of diabetic retinopathy in type 2 diabetes mellitus},
  author={Crosby-Nwaobi, Roxanne and Heng, Ling Zhi and Sivaprasad, Sobha},
  journal={Ophthalmologica},
  volume={228},
  number={2},
  pages={84--92},
  year={2012},
  publisher={Karger Publishers}
}

@article{habib2014association,
  title={The association between retinal vascular geometry changes and diabetic retinopathy and their role in prediction of progression--an exploratory study},
  author={Habib, Maged S and Al-Diri, Bashir and Hunter, Andrew and Steel, David HW},
  journal={BMC Ophthalmology},
  volume={14},
  number={1},
  pages={1--11},
  year={2014},
  publisher={BioMed Central}
}

@INPROCEEDINGS{Howard2019MobileNet,
  author={Howard, Andrew and Sandler, Mark and Chen, Bo and Wang, Weijun and Chen, Liang-Chieh and Tan, Mingxing and Chu, Grace and Vasudevan, Vijay and Zhu, Yukun and Pang, Ruoming and Adam, Hartwig and Le, Quoc},
  booktitle={IEEE/CVF International Conference on Computer Vision (ICCV)}, 
  title={Searching for {MobileNetV3}}, 
  year={2019},
  pages={1314-1324},
  doi={10.1109/ICCV.2019.00140}}

@ARTICLE{Romera2018ERFNet,
  author={Romera, Eduardo and Álvarez, José M. and Bergasa, Luis M. and Arroyo, Roberto},
  journal={IEEE Transactions on Intelligent Transportation Systems}, 
  title={{ERFNet}: Efficient Residual Factorized ConvNet for Real-Time Semantic Segmentation}, 
  year={2018},
  volume={19},
  number={1},
  pages={263-272},
  doi={10.1109/TITS.2017.2750080}}

@Comment{jabref-meta: databaseType:bibtex;}

@Comment{jabref-meta: grouping:
0 AllEntriesGroup:;
1 StaticGroup:Markings\;2\;1\;\;\;\;;
2 StaticGroup:[tariq:]\;2\;1\;\;\;\;;
2 StaticGroup:tariq:6\;2\;1\;\;\;\;;
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
@article{liu2015parsenet,
  title={{ParseNet}: Looking Wider to See Better},
  author={Liu, Wei and Rabinovich, Andrew and Berg, Alexander C},
  journal={arXiv:1506.04579},
  year={2015}
}

@ARTICLE{9910402,
  author={Arsalan, Muhammad and Khan, Tariq M. and Naqvi, Syed S. and Nawaz, Mehmood and Razzak, Imran},
  journal={IEEE/ACM Transactions on Computational Biology and Bioinformatics}, 
  title={Prompt Deep Light-weight Vessel Segmentation Network {(PLVS-Net)}}, 
  year={2022},
  volume={},
  number={},
  pages={1-9},
  doi={10.1109/TCBB.2022.3211936}}
  
@article{Naqvi2023,
   author = {Syed S Naqvi and Zubair Akhtar Langah and Haroon Ahmed Khan and Majid Iqbal Khan and Tariq Bashir and M I Razzak and Tariq M Khan},
   doi = {10.1007/s12559-023-10131-w},
   issn = {1866-9964},
   journal = {Cognitive Computation},
   title = {{GLAN}: GAN Assisted Lightweight Attention Network for Biomedical Imaging Based Diagnostics},
   url = {https://doi.org/10.1007/s12559-023-10131-w},
   year = {2023},
}

@article{Khan2022,
   author = {Tariq M Khan and Syed S Naqvi and Erik Meijering},
   doi = {10.1038/s41598-022-26482-7},
   issn = {2045-2322},
   issue = {1},
   journal = {Scientific Reports},
   pages = {22286},
   title = {Leveraging image complexity in macro-level neural network design for medical image segmentation},
   volume = {12},
   url = {https://doi.org/10.1038/s41598-022-26482-7},
   year = {2022},
}

@inproceedings{khan2020semantically,
  title={A Semantically Flexible Feature Fusion Network for Retinal Vessel Segmentation},
  author={Khan, Tariq M and Robles-Kelly, Antonio and Naqvi, Syed S},
  booktitle={International Conference on Neural Information Processing},
  pages={159--167},
  year={2020}
}
@inproceedings{khan2021residual,
  title={Residual Multiscale Full Convolutional Network ({RM-FCN}) for High Resolution Semantic Segmentation of Retinal Vasculature},
  author={Khan, Tariq M and Robles-Kelly, Antonio and Naqvi, Syed S and Muhammad, Arsalan},
  booktitle={Structural, Syntactic, and Statistical Pattern Recognition: Joint IAPR International Workshops},
  pages={324},
  year={2021}
}
@inproceedings{khan2021rc,
  title={{RC-Net}: A Convolutional Neural Network for Retinal Vessel Segmentation},
  author={Khan, Tariq M and Robles--Kelly, Antonio and Naqvi, Syed S},
  booktitle={Digital Image Computing: Techniques and Application (DICTA)},
  pages={1--7},
  year={2021}
}
@inproceedings{khan2022t,
  title={{T-Net}: A resource-constrained tiny convolutional neural network for medical image segmentation},
  author={Khan, Tariq M and Robles-Kelly, Antonio and Naqvi, Syed S},
  booktitle={IEEE/CVF Winter Conference on Application of Computer Vision (WACV)},
  pages={644--653},
  year={2022}
}
@inproceedings{long2015fully,
  title={Fully Convolutional Networks for Semantic Segmentation},
  author={Long, Jonathan and Shelhamer, Evan and Darrell, Trevor},
  booktitle={IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={3431--3440},
  year={2015}
}
@article{chen2017rethinking,
  title={Rethinking Atrous Convolution for Semantic Image Segmentation},
  author={Chen, Liang-Chieh and Papandreou, George and Schroff, Florian and Adam, Hartwig},
  journal={arXiv:1706.05587},
  year={2017}
}
@article{chen2017deeplab,
  title={{DeepLab}: Semantic Image Segmentation with Deep Convolutional Nets, Atrous Convolution, and Fully Connected {CRF}s},
  author={Chen, Liang-Chieh and Papandreou, George and Kokkinos, Iasonas and Murphy, Kevin and Yuille, Alan L},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  volume={40},
  number={4},
  pages={834--848},
  year={2017},
  publisher={IEEE}
}
@article{gu2019net,
  title={{CE-Net}: Context Encoder Network for {2D} Medical Image Segmentation},
  author={Gu, Zaiwang and Cheng, Jun and Fu, Huazhu and Zhou, Kang and Hao, Huaying and Zhao, Yitian and Zhang, Tianyang and Gao, Shenghua and Liu, Jiang},
  journal={IEEE Transactions on Medical Imaging},
  volume={38},
  number={10},
  pages={2281--2292},
  year={2019},
  publisher={IEEE}
}
@article{zhou2019high,
  title={High-Resolution Encoder-Decoder Networks for Low-Contrast Medical Image Segmentation},
  author={Zhou, Sihang and Nie, Dong and Adeli, Ehsan and Yin, Jianping and Lian, Jun and Shen, Dinggang},
  journal={IEEE Transactions on Image Processing},
  volume={29},
  pages={461--475},
  year={2019},
  publisher={IEEE}
}
@article{zhou2019unet,
  title={{UNet++}: Redesigning Skip Connections to Exploit Multiscale Features in Image Segmentation},
  author={Zhou, Zongwei and Siddiquee, Md Mahfuzur Rahman and Tajbakhsh, Nima and Liang, Jianming},
  journal={IEEE Transactions on Medical Imaging},
  volume={39},
  number={6},
  pages={1856--1867},
  year={2019},
  publisher={IEEE}
}
@article{chen2021transunet,
  title={{TransUNet}: Transformers Make Strong Encoders for Medical Image Segmentation},
  author={Chen, Jieneng and Lu, Yongyi and Yu, Qihang and Luo, Xiangde and Adeli, Ehsan and Wang, Yan and Lu, Le and Yuille, Alan L and Zhou, Yuyin},
  journal={arXiv:2102.04306},
  year={2021}
}
@article{simonyan2014very,
  title={Very Deep Convolutional Networks for Large-Scale Image Recognition},
  author={Simonyan, Karen and Zisserman, Andrew},
  journal={arXiv:1409.1556},
  year={2014}
}
@inproceedings{he2016deep,
  title={Deep Residual Learning for Image Recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={770--778},
  year={2016}
}
@inproceedings{valanarasu2021medical,
  title={Medical Transformer: Gated Axial-Attention for Medical Image Segmentation},
  author={Valanarasu, Jeya Maria Jose and Oza, Poojan and Hacihaliloglu, Ilker and Patel, Vishal M},
  booktitle={International Conference on Medical Image Computing and Computer-Assisted Intervention (MICCAI)},
  pages={36--46},
  year={2021}
}
@inproceedings{hu2018squeeze,
  title={Squeeze-and-Excitation Networks},
  author={Hu, Jie and Shen, Li and Sun, Gang},
  booktitle={IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={7132--7141},
  year={2018}
}
@article{le2019classifying,
  title={Classifying Promoters by Interpreting the Hidden Information of {DNA} Sequences via Deep Learning and Combination of Continuous FastText {N}-Grams},
  author={Le, Nguyen Quoc Khanh and Yapp, Edward Kien Yee and Nagasundaram, N and Yeh, Hui-Yuan},
  journal={Frontiers in Bioengineering and Biotechnology},
  pages={305},
  year={2019},
  publisher={Frontiers}
}

@inproceedings{ni2019raunet,
  title={{RAUNet}: Residual Attention {U-Net} for Semantic Segmentation of Cataract Surgical Instruments},
  author={Ni, Zhen-Liang and Bian, Gui-Bin and Zhou, Xiao-Hu and Hou, Zeng-Guang and Xie, Xiao-Liang and Wang, Chen and Zhou, Yan-Jie and Li, Rui-Qi and Li, Zhen},
  booktitle={International Conference on Neural Information Processing},
  pages={139--149},
  year={2019}
}
@article{li2021pyconvu,
  title={{PyConvU-Net}: A lightweight and multiscale network for biomedical image segmentation},
  author={Li, Changyong and Fan, Yongxian and Cai, Xiaodong},
  journal={BMC Bioinformatics},
  volume={22},
  number={1},
  pages={1--11},
  year={2021}
}
@inproceedings{milletari2016v,
  title={{V-Net}: Fully Convolutional Neural Networks for Volumetric Medical Image Segmentation},
  author={Milletari, Fausto and Navab, Nassir and Ahmadi, Seyed-Ahmad},
  booktitle={IEEE International Conference on 3D vision (3DV)},
  pages={565--571},
  year={2016}
}
@article{xia2017w,
  title={{W-Net}: A Deep Model for Fully Unsupervised Image Segmentation},
  author={Xia, Xide and Kulis, Brian},
  journal={arXiv:1711.08506},
  year={2017}
}
@inproceedings{mehta2017m,
  title={{M-Net}: A Convolutional Neural Network for deep brain structure segmentation},
  author={Mehta, Raghav and Sivaswamy, Jayanthi},
  booktitle={IEEE International Symposium on Biomedical Imaging (ISBI)},
  pages={437--440},
  year={2017}
}

@inproceedings{wong2019segnas3d,
  title={{SegNAS3D}: Network Architecture Search with Derivative-Free Global Optimization for {3D} Image Segmentation},
  author={Wong, Ken C L and Moradi, Mehdi},
  booktitle={Medical Image Computing and Computer-Assisted Intervention (MICCAI)},
  pages={393--401},
  year={2019}
}
@article{nekrasov2018light,
  title={Light-Weight {RefineNet} for Real-Time Semantic Segmentation},
  author={Nekrasov, Vladimir and Shen, Chunhua and Reid, Ian},
  journal={arXiv:1810.03272},
  year={2018}
}
@inproceedings{lin2017refinenet,
  title={{RefineNet}: Multi-Path Refinement Networks for High-Resolution Semantic Segmentation},
  author={Lin, Guosheng and Milan, Anton and Shen, Chunhua and Reid, Ian},
  booktitle={IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={1925--1934},
  year={2017}
}
@inproceedings{zhao2018icnet,
  title={{ICNet} for Real-Time Semantic Segmentation on High-Resolution Images},
  author={Zhao, Hengshuang and Qi, Xiaojuan and Shen, Xiaoyong and Shi, Jianping and Jia, Jiaya},
  booktitle={European Conference on Computer Vision (ECCV)},
  pages={405--420},
  year={2018}
}
@inproceedings{yu2018bisenet,
  title={{BiSeNet}: Bilateral Segmentation Network for Real-time Semantic Segmentation},
  author={Yu, Changqian and Wang, Jingbo and Peng, Chao and Gao, Changxin and Yu, Gang and Sang, Nong},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  pages={325--341},
  year={2018}
}
@article{yu2021bisenet,
  title={{BiSeNet V2}: Bilateral Network with Guided Aggregation for Real-time Semantic Segmentation},
  author={Yu, Changqian and Gao, Changxin and Wang, Jingbo and Yu, Gang and Shen, Chunhua and Sang, Nong},
  journal={International Journal of Computer Vision},
  volume={129},
  number={11},
  pages={3051--3068},
  year={2021},
  publisher={Springer}
}
@article{yuan2019dmfnet,
  title={{DMFNet}: Deep Multi-Modal Fusion Network for {RGB-D} Indoor Scene Segmentation},
  author={Yuan, Jianzhong and Zhou, Wujie and Luo, Ting},
  journal={IEEE Access},
  volume={7},
  pages={169350--169358},
  year={2019},
  publisher={IEEE}
}
@inproceedings{chollet2017xception,
  title={{Xception}: Deep Learning with Depthwise Separable Convolutions},
  author={Chollet, Fran{\c{c}}ois},
  booktitle={IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={1251--1258},
  year={2017}
}
@article{howard2017mobilenets,
  title={{MobileNets}: Efficient Convolutional Neural Networks for Mobile Vision Applications},
  author={Howard, Andrew G and Zhu, Menglong and Chen, Bo and Kalenichenko, Dmitry and Wang, Weijun and Weyand, Tobias and Andreetto, Marco and Adam, Hartwig},
  journal={arXiv:1704.04861},
  year={2017}
}

@article{zhang2020dense,
  title={{DENSE-INception U-net for medical image segmentation}},
  author={Zhang, Ziang and Wu, Chengdong and Coleman, Sonya and Kerr, Dermot},
  journal={Computer Methods and Programs in Biomedicine},
  volume={192},
  pages={105395},
  year={2020}
}
@inproceedings{zhang2018shufflenet,
  title={{ShuffleNet}: An Extremely Efficient Convolutional Neural Network for Mobile Devices},
  author={Zhang, Xiangyu and Zhou, Xinyu and Lin, Mengxiao and Sun, Jian},
  booktitle={IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={6848--6856},
  year={2018}
}
@inproceedings{ma2018shufflenet,
  title={{ShuffleNet V2}: Practical Guidelines for Efficient {CNN} Architecture Design},
  author={Ma, Ningning and Zhang, Xiangyu and Zheng, Hai-Tao and Sun, Jian},
  booktitle={European Conference on Computer Vision (ECCV)},
  pages={116--131},
  year={2018}
}
@article{isensee2021nnu,
  title={{nnU-Net}: a self-configuring method for deep learning-based biomedical image segmentation},
  author={Isensee, Fabian and Jaeger, Paul F and Kohl, Simon AA and Petersen, Jens and Maier-Hein, Klaus H},
  journal={Nature Methods},
  volume={18},
  number={2},
  pages={203--211},
  year={2021},
  publisher={Nature Publishing Group}
}
@inproceedings{lei2020lightweight,
  title={{Lightweight V-Net} for Liver Segmentation},
  author={Lei, Tao and Zhou, Wenzheng and Zhang, Yuxiao and Wang, Risheng and Meng, Hongying and Nandi, Asoke K},
  booktitle={IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={1379--1383},
  year={2020}
}
@inproceedings{tarasiewicz2020lightweight,
  title={{Lightweight U-Nets} for Brain Tumor Segmentation},
  author={Tarasiewicz, Tomasz and Kawulok, Michal and Nalepa, Jakub},
  booktitle={International MICCAI Brain Lesion Workshop},
  pages={3--14},
  year={2020}
}
@article{khan2019review,
  title={{A review of retinal blood vessels extraction techniques: challenges, taxonomy, and future trends}},
  author={Khan, Khan Bahadar and Khaliq, Amir A and Jalil, Abdul and Iftikhar, Muhammad Aksam and Ullah, Najeeb and Aziz, Muhammad Waqar and Ullah, Kifayat and Shahid, Muhammad},
  journal={Pattern Analysis and Applications},
  volume={22},
  number={3},
  pages={767--802},
  year={2019},
  publisher={Springer}
}
@article{franklin2014computerized,
  title={{Computerized screening of diabetic retinopathy employing blood vessel segmentation in retinal images}},
  author={Franklin, S Wilfred and Rajan, S Edward},
  journal={Biocybernetics and Biomedical Engineering},
  volume={34},
  number={2},
  pages={117--124},
  year={2014},
  publisher={Elsevier}
}

@ARTICLE{10049997,
  author={Guo, Erjian and Fu, Huazhu and Zhou, Luping and Xu, Dong},
  journal={IEEE Transactions on Medical Imaging}, 
  title={Bridging Synthetic and Real Images: A Transferable and Multiple Consistency aided Fundus Image Enhancement Framework}, 
  year={2023},
  volume={},
  number={},
  pages={},
  doi={10.1109/TMI.2023.3247783}}

  
@inproceedings{guo2019dynamic,
  title={Dynamic Recursive Neural Network},
  author={Guo, Qiushan and Yu, Zhipeng and Wu, Yichao and Liang, Ding and Qin, Haoyu and Yan, Junjie},
  booktitle={IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={5147--5156},
  year={2019}
}
@article{Lyu2022,
   author = {Xingzheng Lyu and Purvish Jajal and Muhammad Zeeshan Tahir and Sanyuan Zhang},
   issn = {2045-2322},
   issue = {1},
   journal = {Scientific Reports},
   pages = {11868},
   title = {{Fractal dimension of retinal vasculature as an image quality metric for automated fundus image analysis systems}},
   volume = {12},
   year = {2022},
}

@article{XU2022695,
title = {{Dual-channel asymmetric convolutional neural network for an efficient retinal blood vessel segmentation in eye fundus images}},
journal = {Biocybernetics and Biomedical Engineering},
volume = {42},
number = {2},
pages = {695-706},
year = {2022},
issn = {0208-5216},
author = {Yanan Xu and Yingle Fan},
keywords = {Retinal blood vessel segmentation, 2D Gabor filter, Convolutional neural network, Dilated convolution, Feature fusion}
}

@inproceedings{han2018image,
  title={{Image Super-Resolution via Dual-State Recurrent Networks}},
  author={Han, Wei and Chang, Shiyu and Liu, Ding and Yu, Mo and Witbrock, Michael and Huang, Thomas S},
  booktitle={Proceedings of the IEEE Conference on CVPR},
  pages={1654--1663},
  year={2018}
}
@inproceedings{alom2018nuclei,
  title={Nuclei Segmentation with Recurrent Residual Convolutional Neural Networks based {U-Net (R2U-Net)}},
  author={Alom, Md Zahangir and Yakopcic, Chris and Taha, Tarek M and Asari, Vijayan K},
  booktitle={IEEE National Aerospace and Electronics Conference (NAECON)},
  pages={228--233},
  year={2018}
}
@inproceedings{wang2019recurrent,
  title={Recurrent {U-Net} for Resource-Constrained Segmentation},
  author={Wang, Wei and Yu, Kaicheng and Hugonot, Joachim and Fua, Pascal and Salzmann, Mathieu},
  booktitle={IEEE/CVF International Conference on Computer Vision (CVPR)},
  pages={2142--2151},
  year={2019}
}
@article{DRIVEdata,
  title={{Ridge-based vessel segmentation in color images of the retina}},
  author={Staal, Joes and Abr{\`a}moff, Michael D and Niemeijer, Meindert and Viergever, Max A and Van Ginneken, Bram},
  journal={IEEE Transactions Medical Imaging},
  volume={23},
  number={4},
  pages={501--509},
  year={2004},
  publisher={IEEE}
}
@article{STAREDataset,
  title={{Locating blood vessels in retinal images by piecewise threshold probing of a matched filter response}},
  author={Hoover, AD and Kouznetsova, Valentina and Goldbaum, Michael},
  journal={IEEE Transactions Medical Imaging},
  volume={19},
  number={3},
  pages={203--210},
  year={2000},
  publisher={IEEE}
}
@article{zhang2020multistage,
  title={A Multistage Refinement Network for Salient Object Detection},
  author={Zhang, Lihe and Wu, Jie and Wang, Tiantian and Borji, Ali and Wei, Guohua and Lu, Huchuan},
  journal={IEEE Transactions on Image Processing},
  volume={29},
  pages={3534--3545},
  year={2020}
}
@article{liu2022wave,
  title={{Wave-Net}: A lightweight deep network for retinal vessel segmentation from fundus images},
  author={Liu, Yanhong and Shen, Ji and Yang, Lei and Yu, Hongnian and Bian, Guibin},
  journal={Computers in Biology and Medicine},
  pages={106341},
  year={2022},
  volume={152},
  publisher={Elsevier}
}
@article{xiang2022towards,
  title={Towards Bi-directional Skip Connections in Encoder-Decoder Architectures and Beyond},
  author={Xiang, Tiange and Zhang, Chaoyi and Wang, Xinyi and Song, Yang and Liu, Dongnan and Huang, Heng and Cai, Weidong},
  journal={Medical Image Analysis},
  volume={78},
  pages={102420},
  year={2022}
}
@article{kingma2014adam,
  title={Adam: A Method for Stochastic Optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv:1412.6980},
  year={2014}
}

@Misc{CHASEDatasetX,
  title = {{{The Child Heart and Health Study in England (CHASE)}}, Accessed on: Oct 14, 2022},
  url   = {http://www.chasestudy.ac.uk/},
}
@article{HRFDataset,
  title={{Retinal vessel segmentation by improved matched filtering: evaluation on a new high-resolution fundus image database}},
  author={Odstrcilik, Jan and Kolar, Radim and Budai, Attila and Hornegger, Joachim and Jan, Jiri and Gazarek, Jiri and Kubena, Tomas and Cernosek, Pavel and Svoboda, Ondrej and Angelopoulou, Elli},
  journal={IET Image Processing},
  volume={7},
  number={4},
  pages={373--383},
  year={2013},
  publisher={IET}
}
@article{IDRiDDataset,
  title={{Indian Diabetic Retinopathy Image Dataset {(IDRiD)}}: A Database for Diabetic Retinopathy Screening Research},
  author={Porwal, Prasanna and Pachade, Samiksha and Kamble, Ravi and Kokare, Manesh and Deshmukh, Girish and Sahasrabuddhe, Vivek and Meriaudeau, Fabrice},
  journal={Data},
  volume={3},
  number={3},
  pages={25},
  year={2018}
}
@inproceedings{xiang2020bio,
  title={{BiO-Net}: Learning Recurrent Bi-directional Connections for Encoder-Decoder Architecture},
  author={Xiang, Tiange and Zhang, Chaoyi and Liu, Dongnan and Song, Yang and Huang, Heng and Cai, Weidong},
  booktitle={Medical Image Computing and Computer-Assisted Intervention (MICCAI)},
  pages={74--84},
  year={2020}
}

@InProceedings{Wu2018,
author="Wu, Y. and Xia, Y. and Song, Y. and Zhang, Y. and Cai, W.",
title="Multiscale Network Followed Network Model for Retinal Vessel Segmentation",
booktitle="Medical Image Computing and Computer Assisted Intervention ",
year="2018",
pages="119--126"
}

@article{iqbal2022g,
  title={{G-Net Light}: A Lightweight Modified {Google Net} for Retinal Vessel Segmentation},
  author={Iqbal, Shahzaib and Naqvi, Syed S and Khan, Haroon A and Saadat, Ahsan and Khan, Tariq M},
  journal={Photonics},
  volume={9},
  number={12},
  pages={923},
  year={2022}
}

@article{zhang2022segvit,
  title={{SegViT}: Semantic Segmentation with Plain Vision Transformers},
  author={Zhang, Bowen and Tian, Zhi and Tang, Quan and Chu, Xiangxiang and Wei, Xiaolin and Shen, Chunhua and Liu, Yifan},
  journal={arXiv:2210.05844},
  year={2022}
}
@article{arsalan2022prompt,
  title={Prompt Deep Light-weight Vessel Segmentation Network {(PLVS-Net)}},
  author={Arsalan, Muhammad and Khan, Tariq M and Naqvi, Syed S and Nawaz, Mehmood and Razzak, Imran},
  journal={IEEE/ACM Transactions on Computational Biology and Bioinformatics},
  year={2022},
  volume={20},
  number={2},
  pages={1363-1371}
}

@article{khan2022mkis,
  title={{MKIS-Net}: A Light-Weight Multi-Kernel Network for Medical Image Segmentation},
  author={Khan, Tariq M and Arsalan, Muhammad and Robles-Kelly, Antonio and Meijering, Erik},
  journal={arXiv:2210.08168},
  year={2022}
}
@article{khan2022leveraging,
  title={Leveraging image complexity in macro-level neural network design for medical image segmentation},
  author={Khan, Tariq M and Naqvi, Syed S and Meijering, Erik},
  journal={Scientific Reports},
  volume={12},
  number={1},
  pages={22286},
  year={2022},
  publisher={Nature Publishing Group UK London}
}

@inproceedings{strudel2021segmenter,
  title={Segmenter: Transformer for Semantic Segmentation},
  author={Strudel, Robin and Garcia, Ricardo and Laptev, Ivan and Schmid, Cordelia},
  booktitle={IEEE/CVF International Conference on Computer Vision (ICCV)},
  pages={7262--7272},
  year={2021}
}
@inproceedings{ranftl2021vision,
  title={Vision Transformers for Dense Prediction},
  author={Ranftl, Ren{\'e} and Bochkovskiy, Alexey and Koltun, Vladlen},
  booktitle={IEEE/CVF International Conference on Computer Vision (ICCV)},
  pages={12179--12188},
  year={2021}
}
@inproceedings{zheng2021rethinking,
  title={Rethinking Semantic Segmentation from a Sequence-to-Sequence Perspective with Transformers},
  author={Sixiao Zheng and Jiachen Lu and Hengshuang Zhao and Xiatian Zhu and Zekun Luo and Yabiao Wang and Yanwei Fu and Jianfeng Feng and Tao Xiang and Philip H.S. Torr and Li Zhang},
  booktitle={IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={6881--6890},
  year={2021}
}
@article{iqbal2022recent,
  title={Recent trends and advances in fundus image analysis: A review},
  author={Iqbal, Shahzaib and Khan, Tariq M and Naveed, Khuram and Naqvi, Syed S and Nawaz, Syed Junaid},
  journal={Computers in Biology and Medicine},
  pages={106277},
  year={2022},
  volume={151},
  publisher={Elsevier}
}
@article{dosovitskiy2020image,
  title={An Image is Worth 16x16 Words: Transformers for Image Recognition at Scale},
  author={Alexey Dosovitskiy and Lucas Beyer and Alexander Kolesnikov and Dirk Weissenborn and Xiaohua Zhai and Thomas Unterthiner and Mostafa Dehghani and Matthias Minderer and Georg Heigold and Sylvain Gelly and Jakob Uszkoreit and Neil Houlsby},
  journal={arXiv:2010.11929},
  year={2020}
} 
@inproceedings{chen2020generative,
  title={{Generative Pretraining From Pixels}},
  author={Chen, Mark and Radford, Alec and Child, Rewon and Wu, Jeffrey and Jun, Heewoo and Luan, David and Sutskever, Ilya},
  booktitle={International Conference on Machine Learning},
  pages={1691--1703},
  year={2020},
  organization={PMLR}
}
@article{oliveira2018retinal,
  title={{Retinal vessel segmentation based on Fully Convolutional Neural Networks}},
  author={Oliveira, Am{\'e}rico and Pereira, S{\'e}rgio and Silva, Carlos A},
  journal={Expert Sys. with Application},
  volume={112},
  pages={229--242},
  year={2018},
  publisher={Elsevier}
}

@ARTICLE{8476171,
  author={Z. {Yan} and X. {Yang} and K. {Cheng}},
  journal={IEEE Journal of Biomedical and Health Informatics}, 
  title={{A Three-Stage Deep Learning Model for Accurate Retinal Vessel Segmentation}}, 
  year={2019},
  volume={23},
  number={4},
  pages={1427-1436},
  doi={10.1109/JBHI.2018.2872813}
  }
@article{kumar2022itermiunet,
  title={{IterMiUnet: A lightweight architecture for automatic blood vessel segmentation}},
  author={Kumar, Ashish and Agrawal, RK and Joseph, Leve},
  journal={arXiv:2208.01485},
  year={2022}
}
@article{guo2022lighteyes,
  title={{LightEyes}: A Lightweight Fundus Segmentation Network for Mobile Edge Computing},
  author={Guo, Song},
  journal={Sensors},
  volume={22},
  number={9},
  pages={3112},
  year={2022}
}

@InProceedings{Wang2019,
  author    = {Wang, B. and Qiu, S. and He H.},
  booktitle = {Medical Image Computing and Computer Assisted Intervention },
  title     = {{Dual Encoding {U}-Net for Retinal Vessel Segmentation}},
  year      = {2019},
}
@inproceedings{Ribeiro2019,
  title={{Ensemble Learning Approaches for Retinal Vessel Segmentation}},
  author={Ribeiro, Alexandrine and Lopes, Ana P and Silva, Carlos A},
  booktitle={Proceedings of Portuguese Meeting on Bioengineering},
  pages={1--4},
  year={2019},
  organization={IEEE}
}
@article{Khan2019b,
author = {Khan, Mohammad A.U. and Khan, Tariq M. and Naqvi, Syed S. and {Aurangzeb Khan}, M.},
issn = {18631711},
journal = {Signal, Image and Video Processing},
number = {8},
pages = {1667--1675},
publisher = {Springer London},
title = {{GGM classifier with multi-scale line detectors for retinal vessel segmentation}},
volume = {13},
year = {2019}
}

@InProceedings{Wu2019,
author={Wu, Y. and Xia, Y. and Song, Y. and Zhang, D. and Liu, D. and Zhang, C. and Cai, W.},
title={{Vessel-Net: Retinal Vessel Segmentation Under Multi-path Supervision}},
booktitle={Medical Image Computing and Computer Assisted Intervention},
year={2019},
pages={264--272}
}

@article{Feng2020,
  title={{CcNet}: A cross-connected convolutional network for segmenting retinal vessels using multi-scale features},
  author={Feng, Shouting and Zhuo, Zhongshuo and Pan, Daru and Tian, Qi},
  journal={Neurocomputing},
  volume={392},
  pages={268--276},
  year={2020}
}
@article{mahapatra2022novel,
  title={{A novel framework for retinal vessel segmentation using optimal improved frangi filter and adaptive weighted spatial FCM}},
  author={Mahapatra, Sakambhari and Agrawal, Sanjay and Mishro, Pranaba K and Pachori, Ram Bilas},
  journal={Computers in Biology and Medicine},
  volume={147},
  pages={105770},
  year={2022},
  publisher={Elsevier}
}
@inproceedings{guo2021sa,
  title={{SA-UNet}: Spatial Attention {U-Net} for Retinal Vessel Segmentation},
  author={Guo, Changlu and Szemenyei, M{\'a}rton and Yi, Yugen and Wang, Wenle and Chen, Buer and Fan, Changqi},
  booktitle={International Conference on Pattern Recognition (ICPR)},
  pages={1236--1242},
  year={2021}
}
@inproceedings{mou2019cs,
  title={{CS-Net}: Channel and Spatial Attention Network for Curvilinear Structure Segmentation},
  author={Mou, Lei and Zhao, Yitian and Chen, Li and Cheng, Jun and Gu, Zaiwang and Hao, Huaying and Qi, Hong and Zheng, Yalin and Frangi, Alejandro and Liu, Jiang},
  booktitle={Medical Image Computing and Computer-Assisted Intervention (MICCAI)},
  pages={721--730},
  year={2019}
}
@article{wu2021scs,
  title={{SCS-Net}: A Scale and Context Sensitive Network for Retinal Vessel Segmentation},
  author={Wu, Huisi and Wang, Wei and Zhong, Jiafu and Lei, Baiying and Wen, Zhenkun and Qin, Jing},
  journal={Medical Image Analysis},
  volume={70},
  pages={102025},
  year={2021},
  publisher={Elsevier}
}
@article{zhang2021collaborative,
  title={Collaborative Network for Super-Resolution and Semantic Segmentation of Remote Sensing Images},
  author={Zhang, Qian and Yang, Guang and Zhang, Guixu},
  journal={IEEE Transactions on Geoscience and Remote Sensing},
  volume={60},
  pages={1--12},
  year={2021},
  publisher={IEEE}
}
@article{SuperVessel,
  journal = {arXiv:2207.13882},
  author = {Hu, Yan and Qiu, Zhongxi and Zeng, Dan and Jiang, Li and Lin, Chen and Liu, Jiang},
  title = {{SuperVessel}: Segmenting High-resolution Vessel from Low-resolution Retinal Image},
  year = {2022},
}

@article{OCE-NET,
  journal = {arXiv:2207.11396},
  author = {Wei, Xinxu and Yang, Kaifu and Bzdok, Danilo and Li, Yongjie},
  title = {Orientation and Context Entangled Network for Retinal Vessel Segmentation},
  year = {2022},
}

@inproceedings{xie2015holistically,
  title={Holistically-Nested Edge Detection},
  author={Xie, Saining and Tu, Zhuowen},
  booktitle={IEEE International Conference on Computer Vision (ICCV)},
  pages={1395--1403},
  year={2015}
}
@inproceedings{fu2016deepvessel,
  title={{DeepVessel}: Retinal Vessel Segmentation via Deep Learning and Conditional Random Field},
  author={Fu, Huazhu and Xu, Yanwu and Lin, Stephen and Kee Wong, Damon Wing and Liu, Jiang},
  booktitle={Medical Image Computing and Computer-Assisted Intervention (MICCAI)},
  pages={132--139},
  year={2016}
}

@article{yan2018joint,
  title={Joint Segment-Level and Pixel-Wise Losses for Deep Learning Based Retinal Vessel Segmentation},
  author={Yan, Zengqiang and Yang, Xin and Cheng, Kwang-Ting},
  journal={IEEE Transactions on Biomedical Engineering},
  volume={65},
  number={9},
  pages={1912--1923},
  year={2018}
}
@article{oktay2018attention, 
  title={{Attention U-Net}: Learning Where to Look for the Pancreas},
  author={Ozan Oktay and Jo Schlemper and Loic Le Folgoc and Matthew Lee and Mattias Heinrich and Kazunari Misawa and Kensaku Mori and Steven McDonagh and Nils Y Hammerla and Bernhard Kainz and Ben Glocker and Daniel Rueckert},
  journal={arXiv:1804.03999},
  year={2018}
}
@article{li2018h,
  title={{H-DenseUNet}: Hybrid Densely Connected {UNet} for Liver and Tumor Segmentation from {CT} Volumes},
  author={Li, Xiaomeng and Chen, Hao and Qi, Xiaojuan and Dou, Qi and Fu, Chi-Wing and Heng, Pheng-Ann},
  journal={IEEE Transactions on Medical Imaging},
  volume={37},
  number={12},
  pages={2663--2674},
  year={2018}
}
@article{yan2018three,
  title={A Three-Stage Deep Learning Model for Accurate Retinal Vessel Segmentation},
  author={Yan, Zengqiang and Yang, Xin and Cheng, Kwang-Ting},
  journal={IEEE Journal of Biomedical and Health Informatics},
  volume={23},
  number={4},
  pages={1427--1436},
  year={2018}
}
@inproceedings{wang2020ctf,
  title={{CTF-Net}: Retinal Vessel Segmentation via Deep Coarse-To-Fine Supervision Network},
  author={Wang, Kun and Zhang, Xiaohong and Huang, Sheng and Wang, Qiuli and Chen, Feiyu},
  booktitle={IEEE International Symposium on Biomedical Imaging (ISBI)},
  pages={1237--1241},
  year={2020}
}
@article{wang2020csu,
  title={{CSU-Net}: A Context Spatial {U-Net} for Accurate Blood Vessel Segmentation in Fundus Images},
  author={Wang, Bo and Wang, Shengpei and Qiu, Shuang and Wei, Wei and Wang, Haibao and He, Huiguang},
  journal={IEEE Journal of Biomedical and Health Informatics},
  volume={25},
  number={4},
  pages={1128--1138},
  year={2020}
}
@article{shaukat2022three,
  title={{Three-Dimensional Semantic Segmentation of Diabetic Retinopathy Lesions and Grading Using Transfer Learning}},
  author={Shaukat, Natasha and Amin, Javeria and Sharif, Muhammad and Azam, Faisal and Kadry, Seifedine and Krishnamoorthy, Sujatha},
  journal={Journal of Personalized Medicine},
  volume={12},
  number={9},
  pages={1454},
  year={2022},
  publisher={MDPI}
}
@article{guo2022carnet,
  title={{CARNet: Cascade attentive RefineNet for multi-lesion segmentation of diabetic retinopathy images}},
  author={Guo, Yanfei and Peng, Yanjun},
  journal={Complex \& Intelligent Systems},
  volume={8},
  number={2},
  pages={1681--1701},
  year={2022},
  publisher={Springer}
}
@inproceedings{foo2020multi,
  title={Multi-Task Learning for Diabetic Retinopathy Grading and Lesion Segmentation},
  author={Foo, Alex and Hsu, Wynne and Lee, Mong Li and Lim, Gilbert and Wong, Tien Yin},
  booktitle={AAAI Conference on Artificial Intelligence},
  pages={13267--13272},
  year={2020}
}

@article{sambyal2020modified,
  title={{Modified U-Net architecture for semantic segmentation of diabetic retinopathy images}},
  author={Sambyal, Nitigya and Saini, Poonam and Syal, Rupali and Gupta, Varun},
  journal={Biocybernetics and Biomedical Engineering},
  volume={40},
  number={3},
  pages={1094--1109},
  year={2020},
  publisher={Elsevier}
}
@article{guo2019seg,
  title={{L-Seg: An end-to-end unified framework for multi-lesion segmentation of fundus images}},
  author={Guo, Song and Li, Tao and Kang, Hong and Li, Ning and Zhang, Yujun and Wang, Kai},
  journal={Neurocomputing},
  volume={349},
  pages={52--63},
  year={2019},
  publisher={Elsevier}
}
@article{mo2018exudate,
  title={{Exudate-based diabetic macular edema recognition in retinal images using cascaded deep residual networks}},
  author={Mo, Juan and Zhang, Lei and Feng, Yangqin},
  journal={Neurocomputing},
  volume={290},
  pages={161--171},
  year={2018},
  publisher={Elsevier}
}
@article{xue2019deep,
  title={Deep membrane systems for multitask segmentation in diabetic retinopathy},
  author={Xue, Jie and Yan, Shuo and Qu, Jianhua and Qi, Feng and Qiu, Chenggong and Zhang, Hongyan and Chen, Meirong and Liu, Tingting and Li, Dengwang and Liu, Xiyu},
  journal={Knowledge-Based Systems},
  volume={183},
  pages={104887},
  year={2019}
}
@article{tan2017automated,
  title={Automated segmentation of exudates, haemorrhages, microaneurysms using single convolutional neural network},
  author={Tan, Jen Hong and Fujita, Hamido and Sivaprasad, Sobha and Bhandary, Sulatha V and Rao, A Krishna and Chua, Kuang Chua and Acharya, U Rajendra},
  journal={Information Sciences},
  volume={420},
  pages={66--76},
  year={2017},
  publisher={Elsevier}
}
@article{zhu2021gdcseg,
  title={{GDCSeg-Net}: General optic disc and cup segmentation network for multi-device fundus images},
  author={Qianlong Zhu and Xinjian Chen and Qingquan Meng and Jiahuan Song and Gaohui Luo and Meng Wang and Fei Shi and Zhongyue Chen and Dehui Xiang and Lingjiao Pan and Zuoyong Li and and Weifang Zhu},
  journal={Biomedical Optics Express},
  volume={12},
  number={10},
  pages={6529--6544},
  year={2021},
  publisher={Optical Society of America}
}

@article{hasan2021drnet,
  title={{DRNet: Segmentation and localization of optic disc and fovea from diabetic retinopathy image}},
  author={Hasan, Md Kamrul and Alam, Md Ashraful and Elahi, Md Toufick E and Roy, Shidhartho and Mart{\'\i}, Robert},
  journal={Artificial Intelligence in Medicine},
  volume={111},
  pages={102001},
  year={2021},
  publisher={Elsevier}
}
@article{jaemin2017retinal,
  title={{Retinal Vessel Segmentation in Fundoscopic Images with Generative Adversarial Networks}},
  author={Jaemin, S and Sang, JP and Kyu-Hwan, J},
  journal={arXiv:1706.09318},
  year={2017}
}
@inproceedings{maninis2016deep,
  title={Deep Retinal Image Understanding},
  author={Maninis, Kevis-Kokitsi and Pont-Tuset, Jordi and Arbel{\'a}ez, Pablo and Gool, Luc Van},
  booktitle={Medical Image Computing and Computer-Assisted Intervention (MICCAI)},
  pages={140--148},
  year={2016}
}
@article{cherukuri2019deep,
  title={{Deep Retinal Image Segmentation With Regularization Under Geometric Priors}},
  author={Cherukuri, Venkateswararao and Bg, Vijay Kumar and Bala, Raja and Monga, Vishal},
  journal={IEEE Transactions on Image Processing},
  volume={29},
  pages={2552--2567},
  year={2019},
  publisher={IEEE}
}
@article{shin2019deep,
  title={{Deep Vessel Segmentation By Learning Graphical Connectivity}},
  author={Shin, Seung Yeon and Lee, Soochahn and Yun, Il Dong and Lee, Kyoung Mu},
  journal={Transactions image analysis},
  volume={58},
  pages={101556},
  year={2019},
  publisher={Elsevier}
}
@inproceedings{laibacher2019m2u,
  title={{M2U-Net}: Effective and Efficient Retinal Vessel Segmentation for Resource-Constrained Environments},
  author={Laibacher, Tim and Weyde, Tillman and Jalali, Sepehr},
  booktitle={IEEE/CVF Conference on Computer Vision and Pattern Recognition Workshops},
  year={2019},
  pages={1-10}
}
@article{guo2022multiple,
  title={{Multiple lesion segmentation in diabetic retinopathy with dual-input attentive RefineNet}},
  author={Guo, Yanfei and Peng, Yanjun},
  journal={Applied Intelligence},
  pages={1--25},
  year={2022},
  publisher={Springer}
}

@inproceedings{zhou2019collaborative,
  title={Collaborative Learning of Semi-Supervised Segmentation and Classification for Medical Images},
  author={Zhou, Yi and He, Xiaodong and Huang, Lei and Liu, Li and Zhu, Fan and Cui, Shanshan and Shao, Ling},
  booktitle={IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={2079--2088},
  year={2019}
}
@article{powers2020evaluation,
  title={{Evaluation: from precision, recall and F-measure to ROC, informedness, markedness and correlation}},
  author={Powers, David MW},
  journal={arXiv:2010.16061},
  year={2020}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
@ARTICLE{Fortunato2010,
  author  = {Fortunato, S.},
  title   = {Community detection in graphs},
  journal = {Phys. Rep.-Rev. Sec. Phys. Lett.}, 
  volume  = {486},
  year    = {2010},
  pages   = {75-174}
}

@ARTICLE{NewmanGirvan2004,
  author  = {Newman, M. E. J. and Girvan, M.},
  title   = {Finding and evaluating community structure in networks},
  journal = {Phys. Rev. E.}, 
  volume  = {69},
  year    = {2004},
  pages   = {026113}
}

@ARTICLE{Vehlowetal2013,
  author  = {Vehlow, C. and Reinhardt, T. and Weiskopf, D.},
  title   = {Visualizing Fuzzy Overlapping Communities in Networks},
  journal = {IEEE Transactions Vision Comput. Graph.}, 
  volume  = {19},
  year    = {2013},
  pages   = {2486-2495}
}

@ARTICLE{Raghavanetal2007,
  author  = {Raghavan, U. and Albert, R. and Kumara, S.},
  title   = {Near linear time algorithm to detect community structures in large-scale networks},
  journal = {Phys. Rev E.}, 
  volume  = {76},
  year    = {2007},
  pages   = {036106}
}

@ARTICLE{SubeljBajec2011a,
  author  = {\v{S}ubelj, L. and Bajec, M.},
  title   = {Robust network community detection using balanced propagation},
  journal = {Eur. Phys. J. B.}, 
  volume  = {81},
  year    = {2011},
  pages   = {353-362}
}

@ARTICLE{Louetal2013,
  author  = {Lou, H. and Li, S. and Zhao, Y.},
  title   = {Detecting community structure using label propagation with weighted coherent neighborhood propinquity},
  journal = {Physica A.}, 
  volume  = {392},
  year    = {2013},
  pages   = {3095-3105}
}

@ARTICLE{Clausetetal2004,
  author  = {Clauset, A. and Newman, M. E. J. and Moore, C.},
  title   = {Finding community structure in very large networks},
  journal = {Phys. Rev. E.}, 
  volume  = {70},
  year    = {2004},
  pages   = {066111}
}

@ARTICLE{Blondeletal2008,
  author  = {Blondel, V. D. and Guillaume, J. L. and Lambiotte, R. and Lefebvre, E.},
  title   = {Fast unfolding of communities in large networks},
  journal = {J. Stat. Mech.-Theory Exp.}, 
  volume  = {2008},
  year    = {2008},
  pages   = {P10008}
}
@inproceedings{ahn2018fast,
  title={Fast, accurate, and lightweight super-resolution with cascading residual network},
  author={Ahn, Namhyuk and Kang, Byungkon and Sohn, Kyung-Ah},
  booktitle={European Conference on Computer Vision (ECCV)},
  pages={252--268},
  year={2018}
}
@ARTICLE{SobolevskyCampari2014,
  author  = {Sobolevsky, S. and Campari, R.},
  title   = {General optimization technique for high-quality community detection in complex networks},
  journal = {Phys. Rev. E.}, 
  volume  = {90},
  year    = {2014},
  pages   = {012811}
}

@ARTICLE{FortunatoBarthelemy2007,
  author  = {Fortunato, S. and Barthelemy, M.},
  title   = {Resolution limit in community detection},
  journal = {Proceedings Natl. Acad. Sci. U. S. A.}, 
  volume  = {104},
  year    = {2007},
  pages   = {36-41}
}

@ARTICLE{SubeljBajec2011b,
  author  = {\v{S}ubelj, L. and Bajec, M.},
  title   = {Unfolding communities in large complex networks: Combining defensive and offensive label propagation for core extraction},
  journal = {Phys. Rev. E.}, 
  volume  = {83},
  year    = {2011},
  pages   = {036103}
}

@ARTICLE{WangLi2013,
  author  = {Wang, X. and Li, J.},
  title   = {Detecting communities by the core-vertex and intimate degree in complex networks},
  journal = {Physica A.}, 
  volume  = {392},
  year    = {2013},
  pages   = {2555-2563}
}

@ARTICLE{Lietal2013,
  author  = {Li, J. and Wang, X. and Eustace, J.},
  title   = {Detecting overlapping communities by seed community in weighted complex networks},
  journal = {Physica A.}, 
  volume  = {392},
  year    = {2013},
  pages   = {6125-6134}
}

@ARTICLE{Fabioetal2013,
  author  = {Fabio, D. R. and Fabio, D. and Carlo, P.},
  title   = {Profiling core-periphery network structure by random walkers},
  journal = {Sci. Rep.}, 
  volume  = {3},
  year    = {2013},
  pages   = {1467}
}

@ARTICLE{Chenetal2013,
  author  = {Chen, Q. and Wu, T. T. and Fang, M.},
  title   = {Detecting local community structure in complex networks based on local degree central nodes},
  journal = {Physica A.}, 
  volume  = {392},
  year    = {2013},
  pages   = {529-537}
}

@ARTICLE{Zhangetal2007,
  author  = {Zhang, S. and Wang, R. and Zhang, X.},
  title   = {Identification of overlapping community structure in complex networks using fuzzy c-means clustering},
  journal = {Physica A.}, 
  volume  = {374},
  year    = {2007},
  pages   = {483-490}
}

@ARTICLE{Nepuszetal2008,
  author  = {Nepusz, T. and Petr\'oczi, A. and N\'egyessy, L. and Bazs\'o, F.},
  title   = {Fuzzy communities and the concept of bridgeness in complex networks},
  journal = {Phys. Rev. E.}, 
  volume  = {77},
  year    = {2008},
  pages   = {016107}
}

@ARTICLE{FabricioLiang2013,
  author  = {Fabricio, B. and Liang, Z.},
  title   = {Fuzzy community structure detection by particle competition and cooperation},
  journal = {Soft Comput.}, 
  volume  = {17},
  year    = {2013},
  pages   = {659-673}
}

@ARTICLE{Sunetal2011,
  author  = {Sun, P. and Gao, L. and Han, S.},
  title   = {Identification of overlapping and non-overlapping community structure by fuzzy clustering in complex networks},
  journal = {Inf. Sci.}, 
  volume  = {181},
  year    = {2011},
  pages   = {1060-1071}
}

@ARTICLE{Wangetal2013,
  author  = {Wang, W. and Liu, D. and Liu, X. and Pan, L.},
  title   = {Fuzzy overlapping community detection based on local random walk and multidimensional scaling},
  journal = {Physica A.}, 
  volume  = {392},
  year    = {2013},
  pages   = {6578-6586}
}

@ARTICLE{Psorakisetal2011,
  author  = {Psorakis, I. and Roberts, S. and Ebden, M. and Sheldon, B.},
  title   = {Overlapping community detection using Bayesian non-negative matrix factorization},
  journal = {Phys. Rev. E.}, 
  volume  = {83},
  year    = {2011},
  pages   = {066114}
}

@CONFERENCE{ZhangYeung2012,
  author  = {Zhang, Y. and Yeung, D.},
  title   = {Overlapping Community Detection via Bounded Nonnegative Matrix Tri-Factorization},
  booktitle = {In Proceedings ACM SIGKDD Conference}, 
  year    = {2012},
  pages   = {606-614}
}

@ARTICLE{Liu2010,
  author  = {Liu, J.},
  title   = {Fuzzy modularity and fuzzy community structure in networks},
  journal = {Eur. Phys. J. B.}, 
  volume  = {77},
  year    = {2010},
  pages   = {547-557}
}

@ARTICLE{Havensetal2013,
  author  = {Havens, T. C. and Bezdek, J. C. and Leckie, C., Ramamohanarao, K. and Palaniswami, M.},
  title   = {A Soft Modularity Function For Detecting Fuzzy Communities in Social Networks},
  journal = {IEEE Transactions Fuzzy Systems}, 
  volume  = {21},
  year    = {2013},
  pages   = {1170-1175}
}

@misc{Newman2013,
  author = {Newman, M. E. J.},
  title  = {Network data},
  howpublished = "\url{http://www-personal.umich.edu/~mejn/netdata/}",
  year = {2013}
}

@ARTICLE{SubeljBajec2012,
  author  = {\v{S}ubelj, L. and Bajec, M.},
  title   = {Ubiquitousness of link-density and link-pattern communities in real-world networks},
  journal = {Eur. Phys. J. B.}, 
  volume  = {85},
  year    = {2012},
  pages   = {1-11}
}

@ARTICLE{Lancichinettietal2008,
  author  = {Lancichinetti, A. and Fortunato, S. and Radicchi, F.},
  title   = {Benchmark graphs for testing community detection algorithms},
  journal = {Phys. Rev. E.}, 
  volume  = {78},
  year    = {2008},
  pages   = {046110}
}

@ARTICLE{Liuetal2014,
  author  = {Liu, W. and Pellegrini, M. and Wang, X.},
  title   = {Detecting Communities Based on Network Topology},
  journal = {Sci. Rep.}, 
  volume  = {4},
  year    = {2014},
  pages   = {5739}
}

@ARTICLE{Danonetal2005,
  author  = {Danon, L. and Diaz-Guilera, A. and Duch, J. and Arenas, A.},
  title   = {Comparing community structure identification},
  journal = {J. Stat. Mech.-Theory Exp.}, 
  volume  = {},
  year    = {2005},
  pages   = {P09008}
}

@ARTICLE{Gregory2011,
  author  = {Gregory, S.},
  title   = {Fuzzy overlapping communities in networks},
  journal = {J. Stat. Mech.-Theory Exp.}, 
  volume  = {},
  year    = {2011},
  pages   = {P02017}
}

@ARTICLE{LancichinettiFortunato2009,
  author  = {Lancichinetti, A. and Fortunato, S.},
  title   = {Benchmarks for testing community detection algorithms on directed and weighted graphs with overlapping communities},
  journal = {Phys. Rev. E.}, 
  volume  = {80},
  year    = {2009},
  pages   = {016118}
}

@CONFERENCE{HullermeierRifqi2009,
  author  = {Hullermeier, E. and Rifqi, M.},
  title   = {A Fuzzy Variant of the Rand Index for Comparing Clustering Structures},
  booktitle = {in Proceedings IFSA/EUSFLAT Conference}, 
  year    = {2009},
  pages   = {1294-1298}
}


@article{iqbal2023robust,
  title={Robust retinal blood vessel segmentation using a patch-based statistical adaptive multi-scale line detector},
  author={Iqbal, Shahzaib and Naveed, Khuram and Naqvi, Syed S and Naveed, Asim and Khan, Tariq M},
  journal={Digital Signal Processing},
  pages={104075},
  year={2023},
  publisher={Elsevier}
}
@article{iqbal2023ldmres,
  title={{LDMRes-Net}: Enabling Real-Time Disease Monitoring through Efficient Image Segmentation},
  author={Iqbal, Shahzaib and Khan, Tariq M and Alhussein, Musaed and Naqvi, Syed S and Usman, Muhammad and Aurangzeb, Khursheed},
  journal={arXiv:2306.06145},
  year={2023}
}
@article{khan2020region,
  title={A region growing and local adaptive thresholding-based optic disc detection},
  author={Khan, Tariq M and Mehmood, Mehwish and Naqvi, Syed S and Butt, Muhammad Fasih Uddin},
  journal={Plos one},
  volume={15},
  number={1},
  pages={e0227566},
  year={2020},
  publisher={Public Library of Science San Francisco, CA USA}
}


@article{naqvi2019automatic,
  title={Automatic optic disk detection and segmentation by variational active contour estimation in retinal fundus images},
  author={Naqvi, Syed S and Fatima, Nayab and Khan, Tariq M and Rehman, Zaka Ur and Khan, M Aurangzeb},
  journal={Signal, Image and Video Processing},
  volume={13},
  pages={1191--1198},
  year={2019},
  publisher={Springer}
}


@article{naveed2021towards,
  title={Towards automated eye diagnosis: An improved retinal vessel segmentation framework using ensemble block matching 3D filter},
  author={Naveed, Khuram and Abdullah, Faizan and Madni, Hussain Ahmad and Khan, Mohammad AU and Khan, Tariq M and Naqvi, Syed Saud},
  journal={Diagnostics},
  volume={11},
  number={1},
  pages={114},
  year={2021},
  publisher={MDPI}
}

@article{khan2023retinal,
  title={Retinal vessel segmentation via a Multi-resolution Contextual Network and adversarial learning},
  author={Khan, Tariq M and Naqvi, Syed S and Robles-Kelly, Antonio and Razzak, Imran},
  journal={Neural Networks},
  year={2023},
  publisher={Elsevier}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
